Visibility Optimization for Surveillance-Evasion Games

We consider surveillance-evasion differential games, where a pursuer must try to constantly maintain visibility of a moving evader. The pursuer loses as soon as the evader becomes occluded. Optimal controls for game can be formulated as a Hamilton-Jacobi-Isaac equation. We use an upwind scheme to compute the feedback value function, corresponding to the end-game time of the differential game. Although the value function enables optimal controls, it is prohibitively expensive to compute, even for a single pursuer and single evader on a small grid. We consider a discrete variant of the surveillance-game. We propose two locally optimal strategies based on the static value function for the surveillance-evasion game with multiple pursuers and evaders. We show that Monte Carlo tree search and self-play reinforcement learning can train a deep neural network to generate reasonable strategies for on-line game play. Given enough computational resources and offline training time, the proposed model can continue to improve its policies and efficiently scale to higher resolutions.

==> chapter-exploration.tex <==


\begin{abstract}
We consider the exploration problem: an agent equipped with a depth sensor must map out a previously unknown environment using as few sensor measurements as possible. We propose an approach based on supervised learning of a greedy algorithm.  We provide a bound on the optimality of the greedy algorithm using submodularity theory.  Using a level set representation, we train a convolutional neural network to determine vantage points that maximize visibility. We show that this method drastically reduces the on-line computational cost and determines a small set of vantage points that solve the problem. This enables us to efficiently produce highly-resolved and topologically accurate maps of complex 3D environments. Unlike traditional next-best-view and frontier-based strategies, the proposed method accounts for geometric priors while evaluating potential vantage points. While existing deep learning approaches focus on obstacle avoidance and local navigation, our method aims at finding near-optimal solutions to the more global exploration problem. We present realistic simulations on 2D and 3D urban environments.
\end{abstract}


\section{Introduction}

We consider the problem of generating a minimal sequence of observing locations
to achieve complete line-of-sight visibility coverage of an environment.  In
particular, we are interested in the case when environment is initially
unknown.  This is particularly useful for autonomous agents to map out unknown,
or otherwise unreachable environments, such as undersea caverns.  Military
personnel may avoid dangerous situations by sending autonomous agents to scout
new territory.  We first assume the environment is known in order to gain
insights.


Consider a domain $\Omega \subseteq \mathbb{R}^d$.  Partition the domain
$\Omega=\free\cup\obs$ into an open set $\free$ representing the free space,
and a closed set $\obs$ of finite obstacles without holes. We will refer to the
$\obs$ as the environment, since it is characterized by the obstacles.
Let $x_i\in\free$ be a vantage point, from which a range sensor,
such as LiDAR, takes omnidirectional measurements $\proj_{x_i}:S^{d-1}\to\mathbb{R}$.
That is, $\proj_{x_i}$ outputs the distance to closest obstacle for each direction in the unit sphere.
One can map the range measurements to the visibility set $\visset_{x_i}$;
points in $\visset_{x_i}$ are visible from $x_i$:

\beq
x \in \visset_{x_i} \text{ if } \|x-x_i\|_2 < \proj_{x_i} \Big( \frac{x-x_i}{\|x-x_i\|_2} \Big) 
\eeq




As more range
measurements are acquired, $\free$ 
can be approximated by the \emph{cumulatively visible set} $\Omega_k$:
\beq \Omega_k = \bigcup_{i=0}^k \mathcal{V}_{x_i} \eeq
By construction, $\Omega_k$ admits partial ordering: $\Omega_{i-1} \subset \Omega_{i}$.
For suitable choices of $x_i$, it is possible that
$ \Omega_n \to \free$
(say, in the Hausdorff distance).
%But it is non-trivial whether there exists a finite number of  vantage points such that
%$\Omega_n = \Omega$.

We aim at determining a \emph{minimal set of vantage points} $\vanpts$ from which
every $x \in \free$ can be seen.
One may formulate a constrained optimization problem and
look for sparse solutions. When the environment is known, we have the \emph{surveillance} problem:
\beq\label{eq:surveillance-problem}
\min_{\vanpts\subseteq \free} \ | \vanpts | ~~~\text{subject to }  \free=\bigcup_{x\in \vanpts} \visset_{x} \ .
\eeq


When the environment is not known apriori, the agent must be careful to avoid collision with obstacles.
New vantage points must be a point that is currently visible. That is, $x_{k+1} \in \Omega_k$.
Define the set of admissible sequences:
\beq
\seqset(\free):=\{ (x_0,\dots,x_{n-1}) \ |\ n\in\mathbb{N},\ x_0\in\free, \ x_{k+1}\in\Omega_k\}.% \text{ for }k=0,\dots,n-1\}.
\eeq
%Let $\vanpts^n=\{x_i\}_{i=1}^n$ be the sequence of $n$ vantage points.
For the unknown environment, we have the \emph{exploration} problem:
\beq\label{eq:exploration-problem}
\min_{\vanpts \in\seqset(\free)} \ |\vanpts| ~~~\text{subject to }  \free=\bigcup_{x\in \vanpts} \visset_{x}.
\eeq
The problem is feasible as long as obstacles do not have holes.



   \begin{figure}[hptb]
      \centering
      \includegraphics[width=2in]{figures/notation_sketch0.pdf} \quad
      \includegraphics[width=2in]{figures/notation_sketch1.pdf}
      \caption{An illustration of the environment. Dashed and dotted lines are the
horizons from $x_0$ and $x_1$, respectively. Their shadow boundary, $B_1$,
is shown in thick, solid blue.  The area of the green region represents
$g(x_1; \Omega_0)$.  }

      \label{fig:setup}
   \end{figure}




\subsection{Related works}

The surveillance problem is related to the art gallery problem in computational
geometry, where the task is to determine the minimum set of guards who can
together observe a polygonal gallery. Vertex guards must be stationed at the
vertices of the polygon, while point guards can be anywhere in
the interior. For simply-connected polygonal scenes, Chv\'atal
showed that $\lfloor n/3 \rfloor$ vertex guards, where $n$ is the number of vertices,
are sometimes necessary and always sufficient \cite{chvatal1975combinatorial}.
For polygonal scenes with $h$ holes, $\lfloor (n+h)/3 \rfloor$ point
guards are sufficient \cite{bjorling1995efficient,hoffmann1991art}. However,
determining the optimal set of observers is NP-complete
\cite{urrutia2000art,o1983some,lee1986computational}.

%\todo{Make sure to mention integer programming works for known environment.}



Goroshin et al. propose an alternating minimization scheme for optimizing the
visibility of $N$ observers \cite{goroshin2011approximate}.
%They suggest gradually incrementing the number of observers while applying this algorithm in order to find an approximately minimal set.  This is very inefficient.
Kang et al. use a system of differential
equations to optimize the location and orientation of $N$ sensors to maximize
surveillance \cite{kang2017optimal}. Both works assume the number of sensors is given.

For the exploration problem, the ``wall-following'' strategy may be used to map
out simple environments \cite{zhang2004experimental}.  LaValle and
Tovar et al.  \cite{tovar2004gap,lavalle2006planning,tovar2007distance} combine
wall-following with a gap navigation tree to keep track of gaps, critical
events which hide a connected region of the environment that is occluded from a
vantage point. Exploration is complete when all gaps have been eliminated.
This approach does not produce any geometric representation of the environment upon completion, due to limited information from gap sensors.

%For robots equipped with range sensors, a class of approaches pick new
A class of approaches pick new
vantage points along shadow boundaries (aka frontiers), the boundary between free
and occluded regions \cite{yamauchi1997frontier}.
Ghosh et al. propose a frontier-based approach for 2D polygonal environments which requires $r+1$ views,
where $r$ is the number of reflex angles \cite{ghosh2008online}.
For general 2D environments, Landa et al.
\cite{landa2006visibility,landa2007robotic,landa2008visibility} use high order
ENO interpolation to estimate curvature, which is then used to determine how
far past the horizon to step. % in order to uncover the most new information.
However, it is not necessarily optimal to pick only points along the shadow
boundary, e.g. when the map is a star-shaped polygon \cite{ghosh2008online}.


Next-best-view algorithms try to find vantage points that maximize a utility
function, consisting of some notion of \emph{information gain} and another
criteria such as path length.  The vantage point does not have to lie along the
shadow boundary.  A common measure of information gain is the volume of \emph{entire}
unexplored region within sensor range that is not occluded by obstacles
\cite{gonzalez2002navigation, bircher2016receding, bircher2018receding,
heng2015efficient}. Surmann et al. count the number of intersections of rays
into the occlusion \cite{surmann2003autonomous}, while Valente et
al. \cite{valente2014information} use
the surface area of the shadow boundary, weighted by the viewing angle from the vantage points,
to define potential information gain. The issue with these heurisitics is
that they are independent of the underlying geometry. % of the obstacles. 
In addition, computing the information gain at each potential vantage point is
costly and another heurisitic is used to determine which points to sample.

%Bircher et al. use an occupancy grid and a geometric random tree %to determine optimal paths in a receding horizon fashion %\cite{bircher2016receding,bircher2018receding}.  Due to high comp
There has been some attempts to incorporate deep learning into the
exploration problem, but they focus on navigation rather than
exploration.
%Bai et al. \cite{bai2017toward} use neural networks to choose an action from a fixed set of moves. 
The approach of Bai et al. \cite{bai2017toward} terminates when there is no
occlusion within view of the agent, even if the global map is still incomplete.
Tai and Liu \cite{tai2016mobile,tai2017virtual,lei2016robot} train agents to
learn obstacle avoidance. %in unknown environments.

Our work uses a gain function to steer a greedy approach, similar to the
next-best-view algorithms. However, our measure of information gain takes the
geometry of the environment into account. By taking advantage of precomputation
via convolutional neural networks, our model learns shape priors for a large
class of obstacles and is efficient at runtime. We use a volumetric
representation which can handle arbitrary geometries in 2D and 3D. Also, we
assume that the sensor range is larger than the domain, which makes the problem
more global and challenging.

%\subsection{Contributions}
%Mention the algorithm is fast

\section{Greedy algorithm}
\label{sec:greedy}
%Although we are interested in the case when the environment is not known a-priori,
%we first assume the environment is known.
%Given an initial position and corresponding observation, where should the agent 
%record the next observation?
%Since the environment is known, one can compute total visible area for all possible
%pairs of vantage points. The difference between this and the initial area is the gain.
%
%For each potential vantage point, the visibility calculation is $\bigo(m^d)$. Repeating
%for every vantage point leads to $\bigo(m^{2d})$ complexity.
%That is, even when the environment is known, computing the optimal greedy vantage point is expensive.
%
%Now suppose the environment is not known. Then subsequent vantage points can only be
%chosen in the currently visible free space. Among those, again the optimal 
%vantage point is the one that maximizes the gain.


%The minimization problem is hard. 
We propose a greedy approach which sequentially determines a new vantage point, $x_{k+1}$, based on the information gathered from all previous vantage points, $x_0,x_1,\cdots, x_{k}$.
The strategy is greedy because $x_{k+1}$ would be a location that \emph{maximizes the information gain}.

For the surveillance problem, the environment is known. We define the \emph{gain} function:
\begin{equation}g(x;\Omega_k) := |   \visset_x  \cup \Omega_k| - |\Omega_k |, \label{gain-func} \end{equation}
i.e. the volume of the region that is visible from $x$ but not from $x_0,x_1,\cdots,x_{k}$.
Note that $g$ depends on $\obs$, which we omit for clarity of notation.
The next vantage point should be chosen to maximize the newly-surveyed volume. We define the greedy surveillance algorithm as:
\begin{equation} x_{k+1} = \arg \max_{x\in \free} g(x;\Omega_k).\label{eq:greedy-surv}\end{equation}
%On a Cartesian grid over the domain $D$, the brute force search is expensive with complexity $\bigo(m^{2d})$ where $m$ is the number of grid points along one dimension.


The problem of exploration is even more challenging since, by definition, the
environment is not known. Subsequent vantage points must lie within the current visible set $\Omega_k$.
The corresponding greedy exploration algorithm is
\begin{equation} x_{k+1} = \arg \max_{x\in \Omega_k} g(x;\Omega_k).\label{eq:greedy-exp}\end{equation}

However, we remark that in practice, one is
typically interested only in a subset $\envsubset$ of all possible environments
$\envset:=\{\obs|\obs\subseteq\mathbb{R}^d\}$.

For example, cities generally follow a grid-like pattern.  Knowing these priors
can help guide our estimate of $g$ for certain types of $\obs$, even when
$\obs$ is unknown initially.

We propose to encode these priors formally into the parameters, $\theta$, of a learned function:
\beq g_\theta(x; \Omega_k, B_k ) \text{ for } \obs \in \envsubset, \eeq
where $B_k$ is the part of $\partial{\Omega}_k$ that may actually lie in the free space $\free$:
\beq
B_k &= \partial \Omega_k \backslash \obs.
\eeq

See Figure \ref{fig:gain} for an example gain function.
We shall demonstrate that while training for $g_\theta$, incorporating the shadow boundaries %as an additional restriction 
helps, in some sense, localize the learning of $g$, and is essential in creating usable $g_\theta$.

   \begin{figure}[hptb]
      \vspace{.8em}
      \centering
      %\includegraphics[height=1.3in,trim={0 0.11in 0 0.11in},clip]{figures/example_gain_map.pdf}
      %\includegraphics[height=1.3in,trim={0 0.11in 0 0.11in},clip]{figures/example_gain_func.pdf}
      \includegraphics[height=1.4in,trim={0 0.11in 0 0.11in},clip]{figures/example_gain_map.pdf}
      \includegraphics[height=1.4in,trim={0 0.11in 0 0.11in},clip]{figures/example_gain_func.pdf}
	  \caption{ Left: the map of a scene consisting of two disks. Right: the
                intensity of the corresponding gain function. The current vantage point is
                shown as the red dot. The location which maximizes the gain function is shown
                as the red {\tt x}.} \label{fig:gain} 
	  \end{figure}


\subsection{A bound for the known environment}
\label{sec:bound-surv}
We present a bound on the optimality of the greedy algorithm, based on
submodularity \cite{krause2014submodular}, a useful property of set functions.
We start with standard definitions.
Let $V$ be a finite set and $f:2^V \to \mathbb{R}$ be a set function which
assigns a value to each subset $S\subseteq V$. 

\begin{definition}{(Monotonicity)}
A set function $f$ is \emph{monotone} if for
every $A\subseteq B \subseteq V$, $$f(A)\le f(B).$$
\end{definition}

\begin{definition}{(Discrete derivative)}
The \emph{discrete derivative} of $f$ at $S$ with respect to $v\in V$
is $$\Delta_f(v|S):= f(S\cup \{v\}) - f(S).$$
\end{definition}

\begin{definition}{(Submodularity)} A set function $f$ is \emph{submodular} if
for every $A\subseteq B\subseteq V$ and $v\in V\setminus B$, 
$$\Delta_f(v|A) \ge \Delta_f(v|B).$$
\end{definition}

In other words, set functions are submodular if they have diminishing returns.
More details and extensions of submodularity can be found in \cite{krause2014submodular}.


Now, suppose the environment $\obs$ is known.
Let $\vanpts$ be the set of vantage points, and let $\visarea(\vanpts)$ be the 
volume of the region visible from $\vanpts$:
\beq
\cumvisset(\vanpts) &:= \bigcup_{x\in\vanpts} \visset_x \\
\visarea(\vanpts) &:= \Big| \cumvisset(\vanpts) \Big|
\eeq

\begin{lemma}{} 
The function $\visarea$ is monotone.
\end{lemma}

\begin{proof}
Consider $A\subseteq B\subseteq \free$. Since $\visarea$ is the cardinality of unions of sets, we have
\beqstar
\visarea(B) &= \Big| \bigcup_{x\in B} \visset_x  \ \Big| \\ 
 &= \Big| \bigcup_{x\in A\cup\{B\setminus A \}} \visset_x  \ \Big| \\ 
 &\ge \Big| \bigcup_{x\in A} \visset_x  \ \Big| \\ 
 &= \visarea(A).
\eeqstar

\end{proof}

\begin{lemma}{} 
The function $\visarea$ is submodular.
\end{lemma}

\begin{proof}
Suppose $A\subseteq B$ and $\{v\} \in \free\setminus B$. By properties of unions and intersections, we have
\beqstar
\visarea(A\cup \{v\}) + \visarea(B) &= \Big| \bigcup_{x\in (A\cup \{v\})} \visset_x  \Big| + \Big| \bigcup_{x\in B} \visset_x  \Big| \\
&\ge \Big| \bigcup_{x\in A\cup \{v\}\cup B} \visset_x  \Big| + \Big| \bigcup_{x\in (A\cup\{v\}) \cap B} \visset_x  \Big| \\
&= \Big| \bigcup_{x\in  B\cup \{v\}} \visset_x  \Big| + \Big| \bigcup_{x\in A} \visset_x  \Big| \\
&= \visarea( B\cup \{v\}) + \visarea(A)\\
\eeqstar
Rearranging, we have
\beqstar
\visarea(A\cup \{v\}) + \visarea(B) &\ge \visarea( B\cup \{v\}) + \visarea(A)\\
\visarea(A\cup \{v\}) - \visarea(A) &\ge \visarea( B\cup \{v\}) - \visarea(B)\\
\Delta_\visarea (v|A) &\ge \Delta_\visarea(v|B).
\eeqstar%
\end{proof}
Submodularity and monotonicity enable a bound which compares the relative
performance of the greedy algorithm to the optimal solution.

%Consider the problem of maximizing a set function subject to constraints on the
%cardinality of the set.
%\beq
%\max_{S\subseteq V} f(S) \text{ subject to } |S| \le k
%\eeq



\begin{theorem}{}
\label{thm:bound-surv}
Let $\vanpts_k^\ast$ be the optimal set of $k$ sensors.
Let $\vanpts_n= \{x_i\}_{i=1}^n$ be the set of $n$ sensors placed using the greedy surveillance algorithm \eqref{eq:greedy-surv}.
Then,
$$\visarea(\vanpts_n) \ge (1-e^{-n/k}) \visarea(\vanpts_k^\ast) .$$
\end{theorem}


\begin{proof}

For $l<n$ we have    
\begin{align}
\visarea(\vanpts_k^\ast) &\le \visarea(\vanpts_k^\ast \cup \vanpts_l) \label{eq:bound-mono}\\ 
&= \visarea(\vanpts_l) + \Delta_\visarea(\vanpts_k^\ast | \vanpts_l) \\
&= \visarea(\vanpts_l) +  \sum_{i=1}^k \Delta_\visarea(x_i^\ast|\vanpts_l \cup\{x_1^\ast,\dots,x_{i-1}^\ast\} ) \\
&\le \visarea(\vanpts_l) +  \sum_{i=1}^k \Delta_\visarea(x_i^\ast|\vanpts_l) \label{eq:bound-sub}\\
&\le \visarea(\vanpts_l) +  \sum_{i=1}^k \visarea(\vanpts_{l+1}) - \visarea(\vanpts_l) \label{eq:bound-greedy} \\
&= \visarea(\vanpts_l)   + k \big[ \visarea(\vanpts_{l+1}) - \visarea(\vanpts_l)  \big].
\end{align}
Line (\ref{eq:bound-mono}) follows from monotonicity, (\ref{eq:bound-sub}) follows from submodularity
of $\visarea$, and (\ref{eq:bound-greedy}) from definition of the greedy algorithm.
   Define $\delta_l := \visarea(\vanpts_k^\ast) - \visarea(\vanpts_l)$, with $\delta_0:=\visarea(\vanpts_k^\ast)$. 
Then 
   \beqstar
   \visarea(\vanpts_k^\ast) - \visarea(\vanpts_l) &\le k \big[ \visarea(\vanpts_{l+1}) - \visarea(\vanpts_l)\big] \\
   \delta_l &\le k \big[ \delta_l - \delta_{l+1}\big] \\
   \delta_l \Big( 1 -  k \Big) &\le - k \delta_{l+1} \\
   \delta_l \Big( 1 -  \frac{1}{k} \Big) &\ge \delta_{l+1} \\
   \eeqstar
  Expanding the recurrence relation with $\delta_n$, we have 
   \beqstar
   \delta_n &\le  \Big( 1 -  \frac{1}{k} \Big) \delta_{n-1}\\
   &\le \Big( 1-\frac{1}{k} \Big)^n \delta_0 \\
   &= \Big( 1-\frac{1}{k} \Big)^n \visarea(\vanpts_k^\ast) \\
   \eeqstar


	Finally, substituting back the definition for $\delta_n$, we have the desired result:
    \begin{align}
    \delta_n \le  \Big( 1-\frac{1}{k} \Big)^n \visarea(\vanpts_k^\ast) \nonumber \\
    \visarea(\vanpts_k^\ast) - \visarea(\vanpts_n) \le  \Big( 1-\frac{1}{k} \Big)^n \visarea(\vanpts_k^\ast) \nonumber \\
    \visarea(\vanpts_k^\ast)\Big( 1- (1-1/k)^n\Big) \le \visarea(\vanpts_n) \nonumber\\
    \visarea(\vanpts_k^\ast)\Big( 1- e^{-n/k} \Big) \le \visarea(\vanpts_n) \label{eq:bound-exp}
    \end{align}
  where (\ref{eq:bound-exp}) follows from the inequality $1-x\le e^{-x}$.
\end{proof}


In particular, if $n=k$, then $(1-e^{-1})\approx 0.63$. 
This means that $k$ steps of the greedy algorithm is guaranteed to cover at least 63\%
of the total volume, if the optimal solution can also be obtained with $k$ steps. When $n=3k$, the greedy algorithm covers at least 95\% of the total volume.
In \cite{nemhauser1978best}, it was shown that no polynomial time algorithm can achieve a better bound.


\subsection{A bound for the unknown environment}
\label{sec:bound-exp}
When the environment is not known, subsequent vantage points must lie within
the current visible set to avoid collision with obstacles:
\beq
x_{k+1} \in \cumvisset(\vanpts_k)
\eeq
Thus, the performance of the exploration algorithm has a strong dependence on the environment
$\obs$ and the initial vantage point $x_1$. We characterize this dependence
using the notion of the \emph{exploration ratio}.

Given an environment $\obs$ and $A\subseteq\free$, consider the ratio of the marginal value of the greedy exploration algorithm, 
to that of the greedy surveillance algorithm:
\beq
\exgap(A) &:= \frac{ \displaystyle{\sup_{x\in \cumvisset(A)}}\Delta_\visarea(x|A ) }{ \displaystyle{ \sup_{x\in\free}} \Delta_\visarea(x|A)}.
\eeq
That is, $\exgap(A)$ characterizes the relative gap (for lack of a better word) caused by the collision-avoidance constraint $x\in\cumvisset(A)$.
Let $A_x =\{A\subseteq \free|x\in A\}$ be the set of vantage points which contain $x$. 
Define the \emph{exploration ratio} as
\beq
\exgap_x &:= \inf_{A\in A_x} \exgap(A).
\eeq

The exploration ratio is the worst-case gap between the two greedy
algorithms, conditioned on $x$.
It helps to provide a bound for the difference between the optimal
solution set of size $k$, and the one prescribed by $n$ steps the greedy exploration algorithm.




\begin{theorem}{}
\label{thm:bound-exp}
Let $\vanpts_k^\ast =\{x_i^\ast\}_{i=1}^k$ be the optimal sequence of $k$ sensors which includes $x_1^\ast=x_1$.
Let $\vanpts_n= \{x_i\}_{i=1}^n$ be the sequence of $n$ sensors placed using the greedy exploration algorithm
\eqref{eq:greedy-exp}.
Then, for $k,n>1$:
$$\visarea(\vanpts_n) \ge \Big[1-\exp \Big({\frac{-(n-1)\exgap_{x_1}}{k-1}}\Big) \Big(1-\frac{\visarea(x_1)}{\visarea(\vanpts_k^\ast)} \Big)    \Big] \visarea(\vanpts_k^\ast) .$$
\end{theorem}

This is reminiscent of Theorem~\ref{thm:bound-surv}, with two subtle differences. 
The $\big[1-\frac{\visarea(x_1)}{\visarea(\vanpts_k^\ast)}\big]$ term accounts for the shared vantage point $x_1$.
If $\visarea(x_1)$ is large, then the exponential term has little effect, since $\visarea(x_1)$ is already close to $\visarea(\vanpts_k^\ast)$. On the other hand, if it is small, then
the exploration ratio $\exgap_{x_1}$ plays a factor.
The idea of the proof is similar, with some subtle differences in algebra to account for the shared vantage point
$x_1$, and the exploration ratio $\exgap_{x_1}$.

\begin{proof}

We have, for $l<n$:
\begin{align}
\visarea(\vanpts_k^\ast) &\le \visarea(\vanpts_k^\ast \cup \vanpts_l) \nonumber\\ 
&= \visarea(\vanpts_l) + \Delta_\visarea(\vanpts_k^\ast | \vanpts_l) \nonumber\\
&= \visarea(\vanpts_l) +  \sum_{i=1}^k \Delta_\visarea(x_i^\ast|\vanpts_l \cup\{x_1^\ast,\dots,x_{i-1}^\ast\} ) \label{eq:bd-exp-tele}\\
&\le \visarea(\vanpts_l) +  \sum_{i=1}^k \Delta_\visarea(x_i^\ast|\vanpts_l) \label{eq:bd-exp-sub}\\
&= \visarea(\vanpts_l) + \Delta_\visarea(x_1^\ast|\vanpts_l) +  \sum_{i=2}^k \Delta_\visarea(x_i^\ast|\vanpts_l) \nonumber\\
&= \visarea(\vanpts_l) + \sum_{i=2}^k \Delta_\visarea(x_i^\ast|\vanpts_l) \label{eq:bd-exp-x1}\\
&\le \visarea(\vanpts_l) +  \sum_{i=2}^k \max_{x\in\free} \Delta_\visarea(x|\vanpts_l) \nonumber\\
&\le \visarea(\vanpts_l) +  \frac{1}{\exgap_{x_1}} \sum_{i=2}^k \max_{x\in\cumvisset(\vanpts_l)} \Delta_\visarea(x|\vanpts_l) \label{eq:bd-exp-gap}\\
&\le \visarea(\vanpts_l) +  \frac{1}{\exgap_{x_1}} \sum_{i=2}^k \visarea(\vanpts_{l+1}) - \visarea(\vanpts_l) \label{eq:bd-exp-greedy} \\
&= \visarea(\vanpts_l)   + \frac{k-1}{\exgap_{x_1}} \big[ \visarea(\vanpts_{l+1}) - \visarea(\vanpts_l)  \big]. \nonumber
\end{align}
Line \eqref{eq:bd-exp-tele} is a telescoping sum, \eqref{eq:bd-exp-sub} follows from submodularity of $\visarea$,
\eqref{eq:bd-exp-x1} uses the fact that $x_1^\ast\in\vanpts_l$,
\eqref{eq:bd-exp-gap} follows from the definition of $\exgap_{x_1}$ and \eqref{eq:bd-exp-greedy} stems from the definition
of the greedy exploration algorithm \eqref{eq:greedy-exp}.

As before, define $\delta_l := \visarea(\vanpts_k^\ast) - \visarea(\vanpts_l)$. However, this time, note
that $\delta_1:=\visarea(\vanpts_k^\ast) - \visarea(\vanpts_1) = \visarea(\vanpts_k^\ast) - \visarea(x_1) $. 
Then 
   \beqstar
   \visarea(\vanpts_k^\ast) - \visarea(\vanpts_l) &\le \frac{k-1}{\exgap_{x_1}} \big[ \visarea(\vanpts_{l+1}) - \visarea(\vanpts_l)\big] \\
   \delta_l &\le \frac{k-1}{\exgap_{x_1}} \big[ \delta_l - \delta_{l+1}\big] \\
   \delta_l \Big( 1 -  \frac{k-1}{\exgap_{x_1}}  \Big) &\le -  \frac{k-1}{\exgap_{x_1}} \delta_{l+1} \\
   \delta_l \Big( 1 -  \frac{\exgap_{x_1}}{k-1} \Big) &\ge \delta_{l+1} \\
   \eeqstar
  Expanding the recurrence relation with $\delta_n$, we have 
   \beqstar
   \delta_n &\le  \Big( 1 -  \frac{\exgap_{x_1}}{k-1} \Big) \delta_{n-1}\\
   &\le \Big( 1-\frac{\exgap_{x_1}}{k-1} \Big)^{n-1} \delta_1 \\
   &= \Big( 1-  \frac{\exgap_{x_1}}{k-1} \Big)^{n-1}  \big[ \visarea(\vanpts_k^\ast) -\visarea(x_1)\big] \\
   \eeqstar
	Now, substituting back the definition for $\delta_n$, we arrive at
    \begin{align}
    \delta_n &\le  \Big( 1-\frac{\exgap_{x_1}}{k-1} \Big)^{n-1} \big[ \visarea(\vanpts_k^\ast)-\visarea(x_1)\big] \nonumber \\
    \visarea(\vanpts_k^\ast) - \visarea(\vanpts_n) &\le  \Big( 1-\frac{\exgap_{x_1}}{k-1} \Big)^{n-1} \big[ \visarea(\vanpts_k^\ast)-\visarea(x_1)\big] \nonumber \\
    \visarea(\vanpts_k^\ast) -\visarea(x_1) -\big[ \visarea(\vanpts_n)-\visarea(x_1)\big]  &\le  \Big( 1-\frac{\exgap_{x_1}}{k-1} \Big)^{n-1} \big[ \visarea(\vanpts_k^\ast)-\visarea(x_1)\big] \nonumber \\
    \big[\visarea(\vanpts_k^\ast) -\visarea(x_1)\big] \Big(1- \big[ 1-\frac{\exgap_{x_1}}{k-1} \big]^{n-1}\Big)  &\le   \big[ \visarea(\vanpts_n)-\visarea(x_1)\big] \nonumber \\
    \big[\visarea(\vanpts_k^\ast) -\visarea(x_1)\big] \Big(1- e^{-\frac{(n-1)\exgap_{x_1}}{k-1}} \Big)  &\le   \big[ \visarea(\vanpts_n)-\visarea(x_1)\big] \nonumber.
    \end{align}

Finally, with some more algebra
\begin{align}
\big[ \visarea(\vanpts_n)-\visarea(x_1)\big] &\ge    \Big(1- e^{-\frac{(n-1)\exgap_{x_1}}{k-1}} \Big) \big[\visarea(\vanpts_k^\ast) -\visarea(x_1)\big] \nonumber \\
\visarea(\vanpts_n) &\ge  \visarea(x_1)  +  \Big(1- e^{-\frac{(n-1)\exgap_{x_1}}{k-1}} \Big) \big[\visarea(\vanpts_k^\ast) -\visarea(x_1)\big] \nonumber \\
\visarea(\vanpts_n) &\ge  \visarea(x_1)  +  \Big(1- e^{-\frac{(n-1)\exgap_{x_1}}{k-1}} \Big) \visarea(\vanpts_k^\ast) - \visarea(x_1) + \visarea(x_1)   e^{-\frac{(n-1)\exgap_{x_1}}{k-1}}   \nonumber \\
\visarea(\vanpts_n) &\ge    \Big(1- e^{-\frac{(n-1)\exgap_{x_1}}{k-1}} \Big) \visarea(\vanpts_k^\ast) + \visarea(x_1)  e^{-\frac{(n-1)\exgap_{x_1}}{k-1}}  \nonumber \\
\visarea(\vanpts_n) &\ge    \Big(1- e^{-\frac{(n-1)\exgap_{x_1}}{k-1}} \big[ 1-\frac{\visarea(x_1)}{\visarea(\vanpts_n^\ast)} \big] \Big) \visarea(\vanpts_k^\ast)  \nonumber.
\end{align}

\end{proof}



\subsubsection*{Exploration ratio example}
We demonstrate an example where $\exgap_{x}$ can be an arbitrarily small
factor that is determined by the geometry of $\free$.
Figure~\ref{fig:alley} depicts an illustration of the setup for the narrow alley environment.
   \begin{figure}[hptb]
      \centering
      \includegraphics[width=.5\textwidth]{figures/alley.pdf}
	  \caption{A map with a narrow alley. Scale exaggerated for illustration.}
		\label{fig:alley} 
	\end{figure}



Consider a domain $\Omega=[0,1]\times[0,1]$ with a thin vertical wall of width $\varepsilon\ll1$,
whose center stretches from $(\frac{3}{2}\varepsilon,0)$ to
$(\frac{3}{2}\varepsilon,1)$. A narrow opening of size
$\varepsilon^2\times\varepsilon$ is centered at
$(\frac{3}{2}\varepsilon,\frac{1}{2})$.  
Suppose $x_1=x_1^\ast=A$ so that 
$$\visarea(\{x_1\})=\varepsilon +\bigo(\varepsilon^2),$$
where the $\varepsilon^2$ factor is due to the small sliver of the narrow alley visible from $A$.
By observation, the optimal solution contains two vantage points. One such solution places $x_2^\ast =C$.
The greedy exploration algorithm can only place $x_2\in\cumvisset(x_1)=[0,\varepsilon]\times[0,1]$.
One possible location is $x_2=B$.
Then, after 2 steps of the greedy algorithm, we have $$\visarea(\vanpts_2)=\varepsilon+\bigo(\varepsilon^2).$$
Meanwhile, the total visible area is $$\visarea(\vanpts_2^\ast)=1-\bigo(\varepsilon)$$ %+\varepsilon^3$.
and the ratio of greedy to optimal area coverage is 
\beq
\label{eq:alley-greedy-ratio-1}
\frac{\visarea(\vanpts_2)}{\visarea(\vanpts_2^\ast)} =\frac{\varepsilon+\bigo(\varepsilon^2)}{1-\bigo(\varepsilon)} =  \bigo(\varepsilon)
\eeq
The exploration ratio is $\exgap_{x_1}=\bigo(\varepsilon^2)$, since
\beq
\max_{x\in\cumvisset(\{x_1\})} \Delta_\visarea(x|\{x_1\})&=\bigo(\varepsilon^2) \\
\max_{x\in\free} \Delta_\visarea(x|\{x_1\})&=1-\bigo(\varepsilon) \\
\eeq
According to the bound, with $k=n=2$, we should have 
\beq
\frac{\visarea(\vanpts_2)}{\visarea(\vanpts_2^\ast)} &\ge  \Big(1- e^{-\frac{(n-1)\exgap_{x_1}}{k-1}} \big[ 1-\frac{\visarea(x_1)}{\visarea(\vanpts_2^\ast)} \big] \Big) \\
&= \Big(1- e^{-\bigo(\varepsilon^2)} \big[ 1-\bigo(\varepsilon) \big] \Big)\\
&= \bigomega(\varepsilon)
\eeq
which reflects what we see in \eqref{eq:alley-greedy-ratio-1}.


On the other hand, if $\vanpts_2=\{C,B\}$ and $\vanpts_2^\ast=\{C,B\}$, we would have
$$\visarea(\{x_1\})=1-\bigo(\varepsilon)$$ and $\exgap_{x_1}=1$,
since both the greedy exploration and surveillance step coincide.
%\beq
%\max_{x\in\cumvisset(\{x_1\})} \Delta_\visarea(x|\{x_1\})&=\varepsilon-\varepsilon^3 \\
%\max_{x\in\free} \Delta_\visarea(x|\{x_1\})&=\varepsilon-\varepsilon^3 \\
%\eeq
According to the bound, with $k=n=2$, we should have 
\beq
\frac{\visarea(\vanpts_2)}{\visarea(\vanpts_2^\ast)} &\ge  \Big(1- e^{-\frac{(n-1)\exgap_{x_1}}{k-1}} \big[ 1-\frac{\visarea(x_1)}{\visarea(\vanpts_n^\ast)} \big] \Big) \\
%&= \Big(1- e^{-1} \big[ 1-\bigo(1) \big] \Big)\\
&\ge 1-\bigo(\varepsilon)
%&= \bigomega(1),
\eeq
which is the case, since $\visarea(\vanpts_2)=\visarea(\vanpts_2^\ast)$.

By considering the first vantage point $x_1$ as part of the bound,
we account for some of the unavoidable uncertainties associated with unknown environments during exploration.


%One can construct environments with many narrow alleys, and create examples where the number of optimal sensors $k\le n/2$.



\subsection{Numerical comparison}
\label{sec:bound-num}
We compare both greedy algorithms on random arrangements of up to 6 circular obstacles. 
Each algorithm starts from the same initial position and runs until all free area is covered.
We record the number of vantage points required over 200 runs for each number of obstacles.

Surprisingly, the exploration algorithm sometimes requires fewer vantage points
than the surveillance algorithm. Perhaps the latter is too aggressive, or perhaps the collision-avoidance
constraint acts as a regularizer.
For example, when there is a single circle, the greedy surveillance algorithm places the
second vantage point $x_2$ on the opposite side of this obstacle. This may lead to two slivers
of occlusion forming of either side of the circle, which will require 2 additional vantage points to cover.
With the greedy exploration algorithm, we do not have this problem, due to the collision-avoidance constraint.
Figure~\ref{fig:circles-135} shows an select example with 1 and 5 obstacles. 
Figure~\ref{fig:circles-histogram} show the histogram of the number of steps needed
for each algorithm. On average, both algorithms require a similar number of steps, but
the exploration algorithm has a slight advantage.

%and how they perform in relation to their respective bounds.
%For a single convex obstacle, 3 vantage points are required [CITE LANDA]
%In general, we do not know the optimal set.
%As a proxy, we compare to the greedy algorithm for the known environment case.

   \begin{figure}[hptb]
      \centering
      \includegraphics[width=.99\textwidth]{figures/circles_known_vs_unknown_001_01.pdf}
      %\includegraphics[width=.95\textwidth]{figures/circles_known_vs_unknown_012_03.pdf}
      \includegraphics[width=.99\textwidth]{figures/circles_known_vs_unknown_015_05.pdf}
	  \caption{Comparing the greedy algorithm for the known (left) and unknown (right) environment on circular obstacles.
               Spikes on each vantage point indicate the ordering, e.g. the initial point has no spike. Gray areas
               are shadows from each vantage point. Lighter regions are visible from more vantage points.}
		\label{fig:circles-135} 
	\end{figure}




   \begin{figure}[hptb]
      \centering
      \includegraphics[height=.93\textheight]{figures/circles_histogram.pdf}
	  \caption{Histogram of number of vantage points needed for the
surveillance (blue) and exploration (orange) greedy algorithms to completely
cover environments consisting up of to 6 circles.}
		\label{fig:circles-histogram} 
	\end{figure}


\section{Learning the gain function}
In this section, we discuss the method for approximating the gain function when the map is not known.
Given the set of previously-visited vantage points, we compute the cumulative visibility
and shadow boundaries. We approximate the gain function by applying the trained
neural network on this pair of inputs, and pick the next point according to
\eqref{eq:greedy-surv}. This procedure repeats until there are no shadow
boundaries or occlusions. %The map is reconstructed as a byproduct.

The data needed for the training and evaluation of $g_\theta$ are computed
using level sets \cite{osher1988fronts,sethian1999level,osher2006level}.
Occupancy grids may be applicable, but we choose level sets since they have proven
to be accurate and robust. In particular, level sets are necessary for subpixel
resolution of shadow boundaries and they allow for efficient visibility
computation, which is crucial when generating the library of training
examples.

%and in particular, the algorithm of \cite{TCOBS:JCP2004} for visibility computation.
The training geometry is embedded by a signed distance function, denoted by $\map$.
For each vantage point $x_i$, the visibility set is represented by the level
set function $\vis(\cdot,x_i)$, which is computed efficiently using the algorithm described in
\cite{tsai2004visibility}.
%Thus, $\mathds{1}_{\mathcal{V}_{x_i}\Omega} = H\big(\psi_{x_i}\big)$, $H$ is the Heaviside function. 

In the calculus of level set functions, unions and intersections of sets are
translated, respectively, into taking maximum and minimum of the corresponding characteristic
functions.  The cumulatively visible sets  $\Omega_k$  are  represented by  the
level set function $ \Psi_k(x)$, which is defined recursively by
\begin{align}
\Psi_0(x) &=\vis(x,{x_0}), \\
\Psi_k(x) &=\max \left\{ \Psi_{k-1}(x), \vis(x,{x_k}) \right\}, \quad k=1,2,\dots
\end{align}
where the max is taken point-wise. Thus we have 
\begin{align}
\free &= \{x|\map(x) >0\},\\
\visset_{x_i} &= \{x|\vis(x,{x_i})>0\},\\
\Omega_k &= \{x|\Psi_k(x) >0\}.
\end{align}
The shadow boundaries $B_k$
are approximated by the "smeared out" function:
\begin{equation} 
b_k(x) := \delta_\varepsilon (\Psi_k) \cdot \left[ 1-H(G_k(x))  \right],
\end{equation}
where $H(x)$ is the Heaviside function and 
\begin{align}
\delta_\varepsilon(x) &= \frac{2}{\varepsilon}  \cos^2\left( \frac{\pi x }{\varepsilon} \right) \cdot \mathds{1}_{[-\frac{\varepsilon}{2},\frac{\varepsilon}{2}]} (x), \\
\graze(x,x_0) &= (x_0-x)^T \cdot \nabla \map(x),\\
G_0 &= \graze(x,x_0),\\
G_k(x) &= \max\{G_{k-1}(x),\graze(x,x_k)\}, \quad k=1,2,\dots
\end{align}

Recall, the shadow boundaries are the portion of the $\partial \Omega_k$ that lie in free space;
the role of $1-H(G_k)$ is to mask out the portion of obstacles that are currently visible from
$\{x_i\}_{i=1}^k$. See Figure~\ref{fig:ls_notation} for an example of $\graze$.
In our implementation, we take
$\varepsilon=3\Delta x$ where $\Delta x$ is the grid node spacing. We refer
the readers to \cite{tsai2005total} for a short review of  relevant
details.



% SURVEILLANCE
When the environment $\obs$ is known, we can compute the gain function exactly
%\begin{equation}g(x; \Omega_k, \Omega) = \int H\Big( \max \big(\Psi_k(\xi), \psi_x(\xi)  \big) - \Psi_k(\xi) \Big) \ d\xi. \end{equation}
\begin{equation}g(x; \Omega_k) = \int H \Big( H\big(\vis(\xi,x)\big) - H\big( \Psi_k(\xi) \big)\Big) \ d\xi. \end{equation}
We remark that the integrand will 
be 1 where the new vantage point uncovers something not previously seen.
Computing $g$ for all $x$ is costly; 
each visibility and volume computation requires $\bigo(m^d)$ operations, and repeating this for all points
in the domain results in $\bigo(m^{2d})$ total flops. %where $m$ is the number of gridpoints in each of $d$ dimensions.
We approximate it with a function ${\tilde g}_\theta$ parameterized
by $\theta$: %for some suitable metric $d$: $$ L(f_\theta,f) = d \Big(f_\theta(x, \Psi_{\Omega_k}; \phi) , f(x, \Psi_{\Omega_k} ; \Omega)  \Big) $$ is minimized.
\beq {\tilde g}_\theta(x; \Psi_k, \map, b_k) \approx g(x; \Omega_k).
\eeq


% EXPLORATION
If the environment is unknown, we directly approximate the gain function
by learning the parameters $\theta$ of a function 
\beq
g_\theta(x;\Psi_k,b_k) \approx  g(x; \Omega_k) H(\Psi_k) 
\eeq
using only the observations as input. Note the $H(\Psi_k)$ factor is needed for
collision avoidance during exploration because it is not known \emph{a priori} whether
an occluded location $y$ is part of an obstacle or free space.  Thus $g_\theta(y)$ must be zero.





\subsection{Training procedure}

We sample the environments uniformly from a library.  For each $\obs$, a sequence of
data pairs is generated and included into the training set $\mathcal{T}$:
\beq \big(\{ \Psi_k, b_k\}, g(x;\Omega_k)H(\Psi_k) \big), \qquad k=0,1,2,\dots.\eeq
%where $g$ is computed by the level set method. 


For a given environment $\obs$, define a path $\vanpts=\{x_i\}_{i=0}^k$
as admissible if $\map(x_0)>0$ and $\Psi_i(x_{i+1})>0$ for $i=0,\dots,k-1$.
That is, it should only contain points in free space and
in the case of exploration, subsequent points must be visible from at least one
of the previous vantage points.
Let $\mathcal{A}$ be the set of admissible paths.
Then training set should ideally include all paths in $\mathcal{A}$. However
this is too costly, since there are $\bigo(m^{kd})$ paths consisting of $k$ steps.
Instead, to generate causally relevant data, we use an $\varepsilon$-greedy
approach: we uniformly sample initial positions. With probability
$\varepsilon$, the next vantage point is chosen randomly from admissible set.
With probability $1-\varepsilon$, the next vantage point is chosen according to
\eqref{eq:greedy-surv}. Figure~\ref{fig:manifold} shows an illustration of the
generation of causal data along the subspace of relevant shapes.

   \begin{figure}[ht]
      \centering
      \includegraphics[width=.98\textwidth]{figures/manifold_figure/manifold.pdf}
	  \caption{Causal data generation along the subspace of relevant shapes.
               Each dot is a data sample corresponding to a sequence of vantage points.}
		\label{fig:manifold} 
	\end{figure}


 


The function $g_\theta$ is
learned by minimizing the empirical loss across all data pairs for each $\obs$
in the training set $\mathcal{T}$:
\beq
\underset{\theta}{\mathrm{argmin}} \ \frac{1}{N}\sum_{\obs \in \mathcal{T} } \sum_k L\Big(g_\theta(x;\Psi_k,b_k), g(x;\Omega_k) H(\Psi_k) \Big),
\eeq
where $N$ is the total number of data pairs. We use the cross entropy loss function:
\beq
 L(p,q)=\int p(x) \log q(x) + (1-p(x)) \log (1-q(x)) \ dx.
\eeq
   

    \begin{figure}[hptb]
       \centering
       %\subfloat[][]{\includegraphics[height=1.5in,trim={0 0.1in 0 0.1in},clip]{figures/seed_52478_austin35_22_2888_1945_1_01_map.pdf}}\quad
       %\subfloat[][]{\includegraphics[height=1.5in,trim={0 0.1in 0 0.1in},clip]{figures/seed_52478_austin35_22_2888_1945_1_01_vis.pdf}}\phantom{testet}\\
       %\subfloat[][]{\includegraphics[height=1.5in,trim={0 0.1in 0 0.1in},clip]{figures/seed_52478_austin35_22_2888_1945_1_01_horizon.pdf}}\quad
       %\subfloat[][]{\includegraphics[height=1.5in,trim={0 0.1in 0 0.1in},clip]{figures/seed_52478_austin35_22_2888_1945_1_01_gain.pdf}}\\
       %\subfloat[][a)]{\includegraphics[height=.25\textheight,trim={0 0.02in 0 0.02in},clip]{figures/seed_01361_austin21_00_0173_3212_4_05_map.pdf}}\quad
       %\subfloat[][b)]{\includegraphics[height=.25\textheight,trim={0 0.02in 0 0.02in},clip]{figures/seed_01361_austin21_00_0173_3212_4_05_vis.pdf}}\phantom{test}\\
       %\subfloat[][c)]{\includegraphics[height=.25\textheight,trim={0.01in 0.02in 0 0.02in},clip]{figures/seed_01361_austin21_00_0173_3212_4_05_horizon.pdf}}\quad
       %\subfloat[][d)]{\includegraphics[height=.25\textheight,trim={0 0.02in 0 0.02in},clip]{figures/seed_01361_austin21_00_0173_3212_4_05_gain.pdf}}\\
       \subfloat[][a)]{\includegraphics[height=.25\textheight,trim={0 0.02in 0 0.02in},clip]{figures/manifold_figure/seed_97126_austin3_22_2454_3639_4_03_map.pdf}}\quad
       \subfloat[][b)]{\includegraphics[height=.25\textheight,trim={0 0.02in 0 0.02in},clip]{figures/manifold_figure/seed_97126_austin3_22_2454_3639_4_03_vis.pdf}}\phantom{test}\\
       \subfloat[][c)]{\includegraphics[height=.25\textheight,trim={0.01in 0.02in 0 0.02in},clip]{figures/manifold_figure/seed_97126_austin3_22_2454_3639_4_03_horizon.pdf}}\quad
       \subfloat[][d)]{\includegraphics[height=.25\textheight,trim={0 0.02in 0 0.02in},clip]{figures/manifold_figure/seed_97126_austin3_22_2454_3639_4_03_gain.pdf}}\\



	   \caption{A training data pair consists of the cumulative visibility and
		shadow boundaries as input, and the gain function as the output. Each sequence of vantage
        points generates a data sample which depends strongly the shapes of the obstacles and shadows. a) The
		underlying map with current vantage points shown in red. b) The cumulative
		visibility of the current vantage points. c) The corresponding shadow
		boundaries. d) The corresponding gain function.}
	   \label{fig:training-data} \end{figure}


\subsection*{Network architecture}

We use convolutional neural networks (CNNs) to approximate the gain function,
which depends on the shape of $\obs$ and the location $x$. CNNs have been
used to approximate functions of shapes effectively in many applications.
Their feedforward evaluations are efficient if the off-line training cost is
ignored.  The gain function $g(x)$ does not depend \emph{directly} on $x$, but
rather, $x$'s visibility of $\free$, with a domain of dependence bounded by
the sensor range. 
%We expect certain translation invariance in the computation of the gain function. 
We employ a fully convolutional
approach for learning $g$, which makes the network applicable to domains of
different sizes. The generalization to 3D is also straight-forward.


We base the architecture of the CNN on U-Net \cite{ronneberger2015u}, which has
had great success in dense inference problems, such as image segmentation. It
aggregates information from various layers in order to have wide receptive
fields while maintaining pixel precision.  The main design choice is to make
sure that the receptive field of our model is sufficient. That is, we want to
make sure that the value predicted at each voxel depends on a sufficiently
large neighborhood.  For efficiency, we use convolution kernels of size $3$ in
each dimension.  By stacking multiple layers, we can achieve large receptive
fields.  Thus the complexity for feedforward computations is linear in the
total number of grid points. %, i.e. $\bigo(m^d)$. 

%with  the constant in front depending on the kernel size ($3^d$), the number of channels (=4), 
%and the number of layers (about ~20 conv layers). 


%\BLUE{The details of the network are boring, but not sure how to go about it, because it probably should be mentioned? Generally a chart is best, but it may be too big to fit here.}

Define a \emph{conv block} as the following layers:
convolution, batch norm, leaky {\tt relu},
stride 2 convolution, batch norm, and leaky {\tt relu}.
Each \emph{conv block} reduces the image size by a factor of 2.
The latter half of the network increases the image size using \emph{deconv blocks}:
bilinear 2x upsampling, convolution, batch norm, and leaky {\tt relu}.

Our 2D network uses 6 \emph{conv blocks} followed by 6 \emph{deconv blocks},
while our 3D network uses 5 of each block.  We choose the number of blocks to
ensure that the receptive field is at least the size of the training images: $128\times128$
and $64\times64\times64$.  The first \emph{conv block} outputs 4 channels.
The number of channels doubles with each \emph{conv block}, and halves with
each \emph{deconv block}.

The network ends with a single channel, kernel of size~1 convolution layer
followed by the sigmoid activation.  This ensures that the network aggregates all
information into a prediction of the correct size and range.

%\todo{Figure}


\section{Numerical results}


We present some experiments to demonstrate the efficacy of our approach. Also, we demonstrate its limitations.
First, we train on $128\times128$ aerial city blocks cropped from INRIA Aerial Image Labeling Dataset \cite{maggiori2017dataset}.
It contains binary images with building labels from several urban areas, including Austin, Chicago, Vienna, and Tyrol.
We train on all the areas except Austin, which we hold out for evaluation.
We call this model {\bf City-CNN}. We train a similar model {\bf NoSB-CNN} on the same training data, but omit the shadow boundary from the input.
Third, we train another model {\bf Radial-CNN}, on synthetically-generated radial maps, such
as the one in Figure \ref{fig:shapes-gain}.

Given a map, we randomly select an initial location.
In order to generate the sequence of vantage points, we apply
\eqref{eq:greedy-surv}, using $g_\theta$ in place of $g$.  Ties are broken by
choosing the closest point to $x_k$.  We repeat this process until there are no
shadow boundaries, the gain function is smaller than $\epsilon$, or the
residual is less than $\delta$,  where the residual is defined as:
% This should be written mathematically when we finalize the notation
\begin{equation} \label{eq:residual}
r = \frac{|\free \setminus \Omega_k| } {|\free| } .
\end{equation}

We compare these against the algorithm which uses the exact gain function,
which we call {\bf Exact}.  We also compare against {\bf Random}, a random
walker, which chooses subsequent vantage points uniformly from the visible
region, and {\bf Random-SB} which samples points uniformly in a small neighborhood
of the shadow boundaries. We analyze the number of steps required to cover the scene and the
residual as a function of the number of steps.
   \begin{figure}[htbp]
      \vspace{.8em}
      \centering
      \includegraphics[height=1.8in]{figures/seed_52478_austin36_67_3489_3103_1_01_pred_gain.pdf}
      \includegraphics[height=1.8in]{figures/seed_52478_austin36_67_3489_3103_1_01_gain.pdf}

	  \caption{Comparison of predicted (left) and exact (right) gain function
		for an Austin map. Although the functions are not identical, the predicted gain
		function peaks in similar locations to the exact gain function, leading to
		similar steps.}
		\label{fig:gain-compare} 
	\end{figure}



Lastly, we present simulation for exploring 3D environments.
Due to the limited availability of datasets, the model, {\bf 3D-CNN}, is
trained using synthetic $64\times64\times64$ voxel images consisting of
tetrahedrons, cylinders, ellipsoids, and cuboids of random positions, sizes,
and orientations.
In the site\footnote{http://visibility.page.link/demo}, the
interested reader may inspect the performance of the {\bf 3D-CNN} in some other
challenging 3D environments.

%It is much harder to gather sufficient realistic urban environments for
%training, so we only train on synthetic shapes.

For our experiments using trained networks, we make use of a CPU-only machine containing
four Intel Core i5-7600 CPU @ 3.50GHz and 8 GB of RAM.
Additionally, we use an Nvidia Tesla K40 GPU with 12 GB of memory for training
and predicting the gain function in 3D scenes.





   \begin{figure}[htb]
      \vspace{.8em}
      \centering
      \includegraphics[height=1.3in]{figures/austin3_00_2914_3284_num_steps.pdf}
      \includegraphics[height=1.3in]{figures/austin3_00_2914_3284_residual.pdf}
      \caption{Distribution of the residual and number of steps generated
across multiple runs over an Austin map. The proposed method is robust against
varying initial conditions. The algorithm reduces the residual to roughly 0.1 \% within
39 steps by using a threshold on the predicted gain function as a termination
condition. }

      \label{fig:city_stats}
   \end{figure}


   \begin{figure}[htpb]
      \centering
      \includegraphics[height=4in,trim={0 0.02in 0 0.02in},clip]{figures/austin3_00_2914_3284_cnn_36.pdf}
      \caption{\label{fig:austin} An example of 36 vantage points (red disks) using {\bf City-CNN} model. White regions are free space while gray regions are occluded. Black borders indicate edges of obstacles.}
   \end{figure}


   \begin{figure}[htb]
      \centering
      \includegraphics[width=4in]{figures/austin2_00_1513_2258_with_random_sb_residual_vs_steps.pdf}

      \caption{Graph showing the decrease in residual over 50 steps among
	   various algorithms starting from the same initial position for an Austin map.
	   Without using shadow boundary information, {\bf NoSB-CNN} can at times be worse than
	   {\bf Random}. Our {\bf City-CNN} model is significantly faster than {\bf Exact}
	   while remaining comparable in terms of residual.}
      \label{fig:comparison}
   \end{figure}



\subsection*{2D city}
The {\bf City-CNN} model works well on 2D Austin maps.
First, we compare the predicted gain function to the exact gain function on a $128\times128$ map, as in Figure \ref{fig:gain-compare}.
Without knowing the underlying map, it is difficult to accurately determine the gain function.
Still, the predicted gain function peaks in locations similar to those in the exact gain function. This results
in similar sequences of vantage points.

\emph{The algorithm is robust to the initial positions.} Figure~\ref{fig:city_stats}
show the distribution of the number of steps and residual across over 800 runs
from varying initial positions over a $512\times512$ Austin map. In practice, using the
shadow boundaries as a stopping criteria can be unreliable.  Due to numerical
precision and discretization effects, the shadow boundaries may never
completely disappear.  Instead, the algorithm terminates when the maximum
predicted gain falls below a certain threshold $\epsilon$. In this example, we
used $\epsilon = 0.1$. Empirically, this strategy is robust. On average, the
algorithm required 33 vantage points to reduce the occluded region to within
0.1\% of the explorable area.

Figure \ref{fig:austin} shows an example sequence consisting of 36 vantage points.
Each subsequent step is generated in under 1 sec using the CPU and instantaneously with a GPU.

Even when the maximizer of the predicted gain function is different from that
of the exact gain function, the difference in gain is negligible.  This is
evident when we see the residuals for {\bf City-CNN} decrease at similar rates
to {\bf Exact}.  Figure \ref{fig:comparison} demonstrates an example of the
residual as a function of the number of steps for one such sequence generated
by these algorithms on a $1024\times1024$ map of Austin.
We see that {\bf City-CNN} performs comparably to {\bf Exact} approach in terms
of residual.  However, {\bf City-CNN} takes 140 secs to generate 50 steps on
the CPU while {\bf Exact}, an $\bigo(m^4)$ algorithm, takes more than 16
hours to produce 50 steps.


%We show distribution of points that are visited. This should be related to the max/min of total visible area at each location.  Compare this to the plot of the area visible from each vantage point.

   



%\subsection{Comparison against next-best-view}

   \begin{figure}[htpb]
	\vspace{.5em}
      \centering
      \includegraphics[height=4in,trim={0 0.02in 0 0.02in},clip]{figures/austin3_00_2914_3284_no_hor_50.pdf}
      \caption{\label{fig:nosb} A sequence of 50 vantage points generated from {\bf NoSB-CNN}. The points cluster near flat edges due to ambiguity and the algorithm becomes stuck. Gray regions without black borders have not been fully explored.}
   \end{figure}


\subsection*{Effect of shadow boundaries}
\emph{The inclusion of the shadow boundaries as input to the CNN is critical for the algorithm to work.}
Without the shadow boundaries, the algorithm cannot distinguish between obstacles and occluded regions.
If an edge corresponds to an occluded region, then choosing a nearby vantage point will 
reduce the residual. However, choosing a vantage point near a flat obstacle will result in no change to the
cumulative visibility. At the next iteration, the input is same as the previous iteration, and the result will be the same;
the algorithm becomes stuck in a cycle. To avoid this, we prevent vantage points from repeating
by zeroing out the gain function at that point and recomputing the argmax.
Still, the vantage points
tend to cluster near flat edges, as in Figure \ref{fig:nosb}. This clustering behavior causes the {\bf NoSB-CNN} model to
be, at times, worse than {\bf Random}. See Figure \ref{fig:comparison} to see how the clustering inhibits the reduction
in the residual.



\subsection*{Effect of shape}

The shape of the obstacles, i.e. $\Omega^c$, used in training affects the gain function predictions.
Figure \ref{fig:shapes-gain} compares the gain functions produced by {\bf City-CNN} and {\bf Radial-CNN}.


    \begin{figure}[phtb]
	\vspace{2em}
       \centering
       \subfloat[][a)]{\includegraphics[height=1.5in,trim={0 0.11in 0 0.11in},clip]{figures/seed_19536_radial_00000_07_map.pdf}}\phantom{filler}\quad
       \subfloat[][b)]{\includegraphics[height=1.5in,trim={0 0.11in 0 0.11in},clip]{figures/seed_19536_radial_00000_07_gain.pdf}}\\
       \subfloat[][c)]{\includegraphics[height=1.5in,trim={0 0.11in 0 0.11in},clip]{figures/seed_19536_radial_00000_07_pred_gain.pdf}}\quad
       \subfloat[][d)]{\includegraphics[height=1.5in,trim={0 0.11in 0 0.11in},clip]{figures/seed_19536_radial_00000_07_pred_gain_radial.pdf}}\\

       \caption{Comparison of gain functions produced with various models on a
radial scene. Naturally, the CNN model trained on radial obstacles best
approximates the true gain function. a) The underlying radial map with vantage
points show in red. b) The exact gain function c)  {\bf City-CNN} predicted
gain function. d) {\bf Radial-CNN} predicted gain function.}


       \label{fig:shapes-gain}
    \end{figure}



   \begin{figure}[htb]
      \centering
      \includegraphics[height=4in,trim={0 0.02in 0 0.02in},clip]{figures/austin3_00_2914_3284_frequency.pdf}
      \caption{\label{fig:frequency} Distribution of vantage points generated by {\bf City-CNN} method from various initial positions. Hot spots are brighter and are visited more frequently since they are essential for completing coverage.}
   \end{figure}


\subsection*{Frequency map}

Here we present one of our studies concerning the exclusivity of
vantage point placements in $\Omega$. We generated sequences of vantage points
starting from over 800 different initial conditions using {\bf City-CNN} model
on a $512\times512$ Austin map. Then, we model each vantage point as a Gaussian with
fixed width, and overlay the resulting distribution on the Austin map in Figure
\ref{fig:frequency}.  This gives us a frequency map of the most recurring
vantage points. These hot spots reveal regions that are more secluded and
therefore, the visibility of those regions is more sensitive to vantage point
selection.
The efficiency of the CNN method
allows us to address many surveillance related
questions for a large collection of relevant geometries.




\subsection*{Art gallery}
Our proposed approach outperforms the computational geometry solution
\cite{o1987art} to the art gallery problem, even though we do not assume the
environment is known.  The key issue with computational geometry approaches is
that they are heavily dependent on the triangulation.
In an extreme  example, consider an art gallery that is a simple convex $\emph{n-gon}$. Even though it is sufficient to place a single vantage point anywhere in the interior of the room, the triangulation-based approach produces a solution with $\lfloor n/3 \rfloor$ vertex guards.

Figure \ref{fig:art-gallery} shows an example gallery consisting of 58 vertices. The computational
geometry approach requires $\lfloor\frac{n}{3}\rfloor=19$ vantage points to completely cover the scene,
even if point guards are used \cite{bjorling1995efficient,hoffmann1991art}.
The gallery contains $r=19$ reflex angles, so the work of \cite{ghosh2008online} requires $r+1=20$ vantage points.
On average, %across various initial positions, 
{\bf City-CNN}
requires only 8 vantage points.

   \begin{figure}[bpt]
      \centering
      \includegraphics[height=2.5in]{figures/enterprise_art_gallery.pdf}
      \includegraphics[height=2.5in]{figures/enterprise_07.pdf}
      \caption{Comparison of the computational geometry approach and the {\bf City-CNN}
approach to the art gallery problem.  The red circles are the vantage points computed by the methods.
Left: A result computed by the computational geometry approach, given the environment.
%provides 3 solutions based on a 3-coloring of the vertices.  The optimal
%solution shown in blue has 19 nodes. Gray lines are edges of the triangulation.
Right: An example sequence of 7 vantage points generated by the {\bf City-CNN}
model. }

      \label{fig:art-gallery}
   \end{figure}



\subsection*{3D environment}

We present a 3D simulation of a 250m$\times$250m environment based on Castle Square Parks in Boston.
Figure \ref{fig:3d-urban} for snapshots of the algorithm in action.
The map is discretized as a level set function on a $768\times768\times64$ voxel grid.
At this resolution, small pillars are accurately reconstructed by our exploration algorithm.
Each step can be generated in 3 seconds using the GPU or 300 seconds using the
CPU. Parallelization of the distance function computation will further reduce the computation time significantly.
A map of this size was previously unfeasible. % under the same computational resource.
%--- the computation of the exact gain function would take weeks.
Lastly, Figure~\ref{fig:3d-pipes} shows snapshots from the exploration of a
more challenging, cluttered 3D scene with many nooks.




\section{Conclusion}
From the perspective of inverse problems, we proposed a greedy algorithm for
autonomous surveillance and exploration. We show that this formulation can be
well-approximated using convolutional neural networks, which learns
geometric priors for a large class of obstacles. The inclusion of shadow
boundaries, computed using the level set method, is crucial for the success of
the algorithm.
One of the advantages of using the gain function \eqref{gain-func}, an
integral quantity, is its stability with respect to noise in positioning and sensor
measurements. In practice, we envision that it can be used in
conjuction with SLAM algorithms \cite{durrant2006simultaneous,
bailey2006simultaneous} for a wide range of real-world applications.

One may also consider $n$-step greedy algorithms, where $n$ vantage points are
chosen simultaneously.  However, being more greedy is not necessarily better.
If the performance metric is the cardinality of the solution set, then it is
not clear that multi-step greedy algorithms lead to smaller solutions. We saw in
section~\ref{sec:greedy} that, even for the single circular obstacle, the greedy
surveillance algorithm may sometimes require more steps than the exploration
algorithm to attain complete coverage.

If the performance metric is based on the rate in which the objective function
increases, then a multi-step greedy approach would be appropriate.  However, on a grid
with $m$ nodes in $d$ dimensions, there are $\bigo(m^{nd})$ possible
combinations.  For each combination, computing the visibility and gain function
requires $\bigo(nm^d)$ cost. In total, the complexity is $\bigo(nm^{d(n+1)})$,
which is very expensive, even when used for offline training of a neural
network. In such cases, it is necessary to selectively sample only the relevant
combinations. One such way to do that, is through a tree search algorithm.
% which we discuss in the next section in the context of differential games.

%See Supplemental Material for a video clip of the exploration process.

   \begin{figure}[htpb]
      \centering
      \includegraphics[width=5in]{figures/3d_urban_0.png}
      \includegraphics[width=5in]{figures/3d_urban_1.png}
      %\includegraphics[width=5in]{figures/3d_urban_2.png}
      %\includegraphics[width=5in]{figures/3d_urban_3.png}
      %\includegraphics[width=5in]{figures/3d_urban_4.png}
      \caption{Snapshots demonstrating the exploration of an initially unknown
3D urban environment using sparse sensor measurements. The red spheres
indicate the vantage point. The gray surface is the reconstruction of the
environment based on line of sight measurements taken from the sequence of
vantage points. New vantage points are computed in virtually real-time using
{\bf 3D-CNN}.}

      \label{fig:3d-urban}
    \end{figure}

   \begin{figure}[thpb]
      \centering
      %\includegraphics[width=5in]{figures/20180511_messy_pipes_limited_range_0.png}
      \includegraphics[width=5in]{figures/20180511_messy_pipes_limited_range_1.png}
      \includegraphics[width=5in]{figures/20180511_messy_pipes_limited_range_2.png}
      %\includegraphics[width=5in]{figures/20180511_messy_pipes_limited_range_3.png}
      \caption{Snapshots of {\bf 3D-CNN} applied to exploration of a cluttered scene.}
      \label{fig:3d-pipes}
    \end{figure}





==> chapter-intro.tex <==
\chapter{Introduction}

As we approach an era of autonomous drones and self-driving cars, it becomes
increasingly important to develop efficient algorithms for path-planning and
data processing.  Depth sensors, such as LiDAR (Light Detection and Ranging),
allow robotic agents to create virtual maps of the scene. Armed with this
information, agents can perform complicated tasks in environments consisting of
multiple obstacles.  We consider two such problems involving line-of-sight
visibility;  two points are visible from one another if there is no obstacle in
the line segment that connects the points. Lastly, we consider point cloud
feature extraction and classification through the use of random rays.

\section{Contributions}
Broadly speaking, we develop mathematical algorithms for various problems
involving visibility. Key components of these algorithms often involve
computationally expensive operations. We apply neural networks to efficiently
approximate those operations. Our success so far seems to be rooted in the
generation of causally relevant data and in the flexibility of neural
networks to interpolate such data.  
%instead of using neural networks to define functions that approximate those components.


In Chapter~\ref{chap:exploration}, we consider the exploration problem: an
agent equipped with a depth sensor must map out a previously unknown
environment using as few sensor measurements as possible. We propose an approach
based on supervised learning of a greedy algorithm.  We provide a bound on the
optimality of the greedy algorithm using submodularity theory.  Using a level
set representation, we train a convolutional neural network to determine
vantage points that maximize visibility. We show that this method drastically
reduces the on-line computational cost and determines a small set of vantage
points that solve the problem. This enables us to efficiently produce
highly-resolved and topologically accurate maps of complex 3D environments.
Unlike traditional next-best-view and frontier-based strategies, the proposed
method accounts for geometric priors while evaluating potential vantage points.
While existing deep learning approaches focus on obstacle avoidance and local
navigation, our method aims at finding near-optimal solutions to the more
global exploration problem. We present realistic simulations on 2D and 3D urban
environments.

In Chapter~\ref{chap:surveillance}, we consider surveillance-evasion
differential games, where a pursuer must try to constantly maintain visibility
of a moving evader.  The pursuer loses as soon as the evader becomes occluded.
Optimal controls for game can be formulated as a Hamilton-Jacobi-Isaac
equation. We use an upwind scheme to compute the feedback value
function, corresponding to the end-game time of the differential game. Although
the value function enables optimal controls, it is prohibitively expensive to
compute, even for a single pursuer and single evader on a small grid. We
consider a discrete variant of the surveillance-game. We propose two locally
optimal strategies based on the static value function for the
surveillance-evasion game with multiple pursuers and evaders. We show that
Monte Carlo tree search and self-play reinforcement learning can train a deep
neural network to generate reasonable strategies for on-line game play. Given
enough computational resources and offline training time, the proposed model
can continue to improve its policies and efficiently scale to higher resolutions.

In Chapter~\ref{chap:raysense}, we present an algorithm for the classification
of point clouds.  The algorithm exploits properties of the point clouds'
signature in  a new framework called \emph{RaySense}.  The RaySense signature
is computed by finding nearest neighbors along a set of randomly generated
rays.  From the signature, statistical information about the whole data set, as
well as certain geometric information, can be extracted, independent of the
choice of ray set.  A RaySense signature is not merely a subset of the point
cloud: while all points sampled by each ray retain some local geometrical
information of the point cloud, certain specific points are sampled repeatedly
by different rays, giving a more global ``sketch'' of the point cloud's shape.
We propose a convolutional neural network, \emph{RayNN}, that uses RaySense
signatures for point cloud classification.  We evaluate RayNN on the 3D
ModelNet benchmark and compare its performance with other state-of-the-art
methods. RayNN results are comparable to other methods, while enjoying lower
complexity.  However, in the presence of additional corruptions, such as the
introduction of unseen outliers or removal of data points, RayNN appears to be
more robust.

%The work in Chapter~\ref{chap:raysense} is part of a preprint completed in collaboration with
%Liangchen Liu and Colin Macdonald from the Department of Mathematics at the University of British Columbia.
%The collaboration initiated at the Institute for Pure and Applied Mathematics
%(IPAM).


\section{Visibility level sets}
We first review our representation of geometry and visibility.
All the functions described below can be computed efficiently in $\bigo(m^d)$, where
$m$ is the number of grid points in each of $d$ dimensions.

\subsection*{Level set functions}
Level set functions \cite{osher1988fronts,sethian1999level,osher2006level} are useful as an implicit
representation of geometry.  Let $\obs \subseteq \mathbb{R}^d$ be a closed set
of a finite number of connected components
representing the obstacle. Denote the occluder function $\map$ with the following properties:
\beq
\begin{cases}
\map(x) < 0 & x \in \obs \\
\map(x) = 0 & x \in \partial \obs \\
\map(x) > 0 & x \notin \obs \\
\end{cases}
\label{eq:occluder}
\eeq

The occluder function is not unique; notice that for any constant $c>0$, the function $c \map$
also satisfies (\ref{eq:occluder}). We use the signed distance function as the occluder function:
\beq
\map(x):= 
\begin{dcases}
-\inf_{y\in \partial \obs} \|x-y\|_2 & x\in \obs \\
\inf_{y\in \partial \obs} \|x-y\|_2 & x \notin \obs
\end{dcases}
\eeq
The signed distance function is a viscosity solution to the Eikonal equation:
\beq
|\nabla \map| &= 1 \\
\map(x) &= 0 \text{ for } x \in \partial \obs
\eeq

It can be computed, for example, using the fast sweeping method \cite{tsai2002rapid} or
the fast marching method \cite{tsitsiklis1995efficient}.



\subsection*{Visibility function}
Let $\free$ be the open set representing free space. Let $\visset_{x_0}$ be the set of points in $\free$
visible from $x_0\in\free$. We seek a function $\vis(x,x_0)$ with properties

\beq
\begin{cases}
\vis(x,y) > 0 & x \in \visset_{x_0} \\
\vis(x,y) = 0 & x \in \partial \visset_{x_0} \\
\vis(x,y) < 0 & x \notin \visset_{x_0} \\
\end{cases}
\label{eq:visibility}
\eeq

Define the visibility level set function $\vis$:
\beq
\vis(x,{x_0}) = \min_{r\in[0,1]} \map(x_0 + r(x-{x_0}))
\eeq

It can be computed efficiently using the fast sweeping method based on the PDE formulation described in \cite{tsai2004visibility}:


\beq
\nabla \vis \cdot \frac{x-{x_0}}{|x-{x_0}|} &= \min \Big\{ H(\vis-\map) \nabla \vis \cdot \frac{x-{x_0}}{|x-{x_0}|},0 \Big\} \\
\vis({x_0},{x_0}) &= \map({x_0})
\eeq
where $H$ is the characteristic function of $[0,\infty)$.



\subsection*{Shadow function}
\label{sec:shadow}
When dealing with visibility, it is useful to represent the shadow regions. 
The gradient of the occluder function $\nabla \map$ is perpendicular to the
level sets $\map$.  The dot product
of $\nabla \map$ and the viewing direction $(x_0-x)$ characterizes the cosine
of the grazing angle $\theta$ between obstacles and viewing direction. In particular,
$|\theta|<\pi/4$ for the portion of obstacles that are directly visible to $x_0$.

Define the grazing function:
\beq
\graze(x,x_0) &= (x_0-x)^T \cdot \nabla \map(x)\\
\eeq

By masking with the occluder function, we can characterize the portion of the
obstacle boundary that is not visible from the vantage point $x_0$.  Define the
auxiliary and auxiliary visibility functions: \beq \aux(x,x_0) &= \max \{
\map(x,x_0), \graze(x,x_0) \} \\ \tilde{\aux}(x,x_0) &= \min_{r\in[0,1]} \aux(x
+ r(x_0-x),x_0) \\ \eeq

By masking the auxilary visibility function with the obstacle, we arrive at the desired
shadow function \cite{takei2014efficient}:
\beq
\shadow(x,x_0) &= \max\{ \tilde{\aux}(x,x_0), -\map(x)\}
\eeq

\captionsetup[subfloat]{labelformat=empty}
\begin{figure}[hptb]
\centering
\subfloat[Occluder function $\map(\cdot)$]{\includegraphics[width=.35\textwidth]{figures/ls_notation_occluder.pdf}} \quad
\subfloat[Visibility function $\vis(\cdot)$]{\includegraphics[width=.35\textwidth]{figures/ls_notation_visibility.pdf}} \\
\subfloat[Grazing function $\graze(\cdot)$]{\includegraphics[width=.35\textwidth]{figures/ls_notation_dot.pdf}} \quad
\subfloat[Auxiliary function $\aux(\cdot)$]{\includegraphics[width=.35\textwidth]{figures/ls_notation_aux.pdf}} \\
\subfloat[Auxiliary visibility function $\tilde{\aux}(\cdot)$]{\includegraphics[width=.35\textwidth]{figures/ls_notation_aux_tilde.pdf}} \quad
\subfloat[Shadow function $\xi(\cdot)$]{\includegraphics[width=.35\textwidth]{figures/ls_notation_shadow.pdf}}
\caption{Level set functions from a vantage point $x_0$ (blue dot). Each function is negative in the shaded region. Obstacle boundary shown as black contour.} \label{fig:ls_notation}

\end{figure}


The difference between the shadow function and the visibility function is that
the shadow function excludes the obstacles.
Although 
$$\tilde{\shadow}(x,x_0) = \max\{-\map(x),\vis(x,x_0)\}$$ 
looks like a candidate shadow function, it 
is not correct. In particular 
$$\{ x|\tilde{\shadow}(x,x_0)=0\}$$ 
includes the portion of the obstacle boundary visible to $x_0$.


Figure~\ref{fig:ls_notation} summarizes the relevant level set functions used in this work.



\section{Convolutional neural networks}
Convolutional neural networks (CNNs) have become the undisputed
state-of-the-art for image classification tasks, where an input image has to be
binned into one of $k$ classes. CNNs are advantageous in that they use a
learned classifier over learned set of features. This has been empirically
shown to be better than the previous state-of-the-art, where learned
classifiers were trained on hand-tuned features. 
Training generally requires lots of data and
computational time.

%CNNs are appealing for image inputs due to their translational equivariance, efficiency, and representational capacity. 


A neural network architecture consists of various layers, which map the input
to the desired output. There are many architectures; the most popular image
classification networks are Alex-Net \cite{krizhevsky2012imagenet} , VGG
\cite{simonyan2014very}, Inception \cite{szegedy2015going}, and ResNet
\cite{he2016deep}.  More recently, fully convolutional neural networks have
shown promise in dense inference tasks, which requires an output for each
input. One such network, U-Net \cite{ronneberger2015u}, is popular due to its
simple architecture and ability to aggregate information across multiple
scales.



\subsection*{Neural networks}
We review some basic concepts. 
A single layer neural network is defined by a function 
\[
y=f(x;W,b):=\mathbf{\sigma}(Wx+b),
\]
where $x\in\mathbb{R}^m$ is the input and $y\in\mathbb{R}^n$ is the output.
The parameters $W$ and $b$ are \emph{learned}, where
$W:\mathbb{R}^{m}\to\mathbb{R}^{n}$ is a linear function; i.e.  an $n\times m$
real-valued matrix, while $b \in \mathbb{R}^{n}$ is a bias term. Lastly,
$\sigma:\mathbb{R}^n\to\mathbb{R}^n$ is a nonlinear activation function.
Common nonlinearities include \emph{sigmoid}: $\sigma(y)=1/(1+e^{-y})$ and
\emph{ReLU}: \mbox{$\sigma(y) = \max\{0,y\}$}.  The activation function is an
``element-wise'' function; i.e. if
$y=(y_{1},y_{2,}\cdots,y_{n})$ , then
$$
\sigma(y):=(\sigma(y_{1}),\sigma(y_{2}),\cdots,\sigma(y_{n})).
$$
For classification tasks, the \emph{softmax} function normalizes the output so that it sums
to $1$:
$$
S(y):=\frac{e^{y}}{\displaystyle \sum_{j=1}^n e^{y_j}}.
$$
%Convolution $\implies$ e.g. W is a tridiagonal matrix for convolution of one dimensional signals
Through the compositions of functions, a neural network can have multiple layers:
\begin{align*}
y^{(L)} & :=f_{L}(f_{L-1}\circ\cdots\circ f_{1}(x,W^{(1)},b^{(1)}),\dots,W^{(L)},b^{(L)})\\
 & \equiv f(x;W^{(1)},\cdots,W^{(L)},b^{(1)},\cdots,b^{(L)}),
\end{align*}
where
\begin{align}
y^{(0)} & :=x \nonumber,\\
y^{(\ell+1)} & :=\sigma_{\ell}(W^{(\ell+1)}y^{(\ell)}+b^{(\ell+1)}),\,\,\,\ell=0,1,\cdots,L-1. \label{eq:nn-recursion}
\end{align}
The function $\sigma_{\ell}$ is the activation function or some
operations that change the dimensionality of a vector for layer $\ell$. 

%The \emph{depth} of a neural network refers to the number of layers $L$. 
\subsection*{Residual networks}
For very deep neural networks with many layers, \cite{he2016deep} showed that
incorporating a \emph{residual~connection} into \eqref{eq:nn-recursion} eases
the training process and improves accuracy.  A \emph{residual connection} with
layer $\ell$ is similar to an explicit Euler scheme -- the operation is an update
to that layer rather than an operation on the entire output of that layer:
\begin{align*}
y^{(\ell+1)} & :=y^{(\ell)}+\sigma_{\ell}(W^{(\ell+1)}y^{(\ell)}+b^{(\ell+1)}),\,\,\,\ell=0,1,\cdots,L-1.
%y^{(0)} & :=x\,\,(\text{the input)}.
\end{align*}



\subsection*{Training}
The parameters $\theta:=(W^{(1)},\cdots,W^{(L))},b^{(1)},\cdots,b^{(L)})$,
are learned via stochastic gradient descent to minimize the \emph{empirical risk}:
\[
%\mathcal{L}(\theta)\equiv\mathcal{L}(\theta;\{(\tilde{x}_{j},\tilde{y}_{j})\}_{j=1}^{N})\stackrel{e.g.}{=}
\frac{1}{N}\sum_{j=1}^{N}\mathcal{L}(\tilde{y}_{j},f(\tilde{x}_{j};\theta)) %+\underbrace{\lambda||\theta||^{2}}_{\text{regularization}},
\]
where $\mathcal{L}$ is the loss function and $(\tilde{x}_{j},\tilde{y}_{j})\}_{j=1}^{N}$ are $N$ training examples.
The loss function is typically the \emph{squared loss} for regression tasks:
\beqstar
\mathcal{L}(p,q) &= \|p-q\|_2^2,
\eeqstar
or the \emph{cross entropy loss} for classification tasks:
\beqstar
\mathcal{L}(p,q) &= -p \cdot \log(q).
\eeqstar

% and the optimal parameters, ideally, would be the minimizer of $\mathcal{L}:$
%\[
%\theta^{*}:=\arg\min_{\theta\in\mathbb{R}^{K}}\mathcal{L}(\theta;\{(\tilde{x}_{j},\tilde{y}_{j})\}_{j=1}^{N}).
%\]
\subsection*{Convolution}
Next, we describe the operations that act on 2D
image-based inputs.  
Generally, the input is a stack of 2D images.  The third
(stack) dimension is the feature dimension.  One can think of each pixel in the
image as a feature vector.  For example, an RGB image has 3 channels, where
each pixel is a vector describing the intensity of red, green, and blue. 

A \emph{convolution} layer convolves the input with a filter, whose weights are
learned. The filter operates on all image channels, but only acts on a small
neighborhood of spatial pixels, determined by the kernel size. Each filter
takes as input a 3D image, and outputs a 2D image.  Each convolutional layer
may have multiple filters, resulting in a 3D stack of filtered images as
output. 

Let  $x\in\mathbb{R}^{M_\text{in}\times N_\text{in}\times D_\text{in}}$ be an
input vector-valued image,
where $M_\text{in}$, $N_\text{in}$, and $D_\text{in}$
are the width, height and number of channels, respectively.
%The output is $y\in\mathbb{R}^{M_{out}\times N_{out}\times D_{out}}$.
Let $s_{k}$ be the kernel size (generally odd so that there is a
well-defined center) and $D_{out}$ be the number of filters. Then
the output of the convolutional layer is 
$y\in\mathbb{R}^{M_{out}\times N_{out}\times D_{out}}$,
where $M_{out}=M_{in}-s_{k}+1$, $N_{out}=N_{in}-s_{k}+1$, and each
entry in $y:=W\ast x+b$ is given by 
\[
y_{ijk}=b_{k}+\sum_{r=1}^{D_{in}}\sum_{q=0}^{s_{k}}\sum_{p=0}^{s_{k}}W_{p,q,r,k} \ x_{i+p,j+q,r}
\]
where $W\in\mathbb{R}^{s_{k}\times s_{k}\times D_{in}\times D_{out}}$
and $b\in\mathbb{R}^{D_{out}}$ is the bias.

In general, a zero padding of $s_{p}$ pixels can be introduced to
the spatial dimensions of the input image to change the output size.
This is particularly useful to make the output image the same size
as the input. Also, a stride of $s_{s}$ pixels can be used if it
is not desirable to apply filter to consecutive pixels. In this case,
$M_{out}=\frac{1}{s_{s}}(M_{in}-s_{k}+2s_{p})+1$ , $N_{out}=\frac{1}{s_{s}}(N_{in}-s_{k}+2s_{p})+1$
and
\[
y_{ijk}=b_{k}+\sum_{r=1}^{D_{in}}\sum_{q=0}^{s_{k}}\sum_{p=0}^{s_{k}}W_{p,q,r,k} \ \tilde{x}_{s_{s}\cdot i+p,s_{s}\cdot j+q,r}
\]
where $\tilde{x}$ is the zero-padded image.
A common choice for kernel size is $s_{k}=3$, with zero padding $s_{p}=1$
and stride $s_{s}=1$. 
%(Although this operation is actually known as correlation in signal processing, the name \emph{convolution} has stuck in the deep learning community).  
%\item \emph{Nonlinearity}: an element-wise nonlinear transformation that
%allows neural networks to learn arbitrary functions. The most commonly
%used is the rectified linear unit, aka ReLU. It is popular due to
%its simplicity and has been shown emprically to improve training over
%other functions, such as the sigmoid or tanh, which suffer from the
%\emph{vanishing gradient} problem. Define $Y:=\text{ReLU}(X)$
%where each entry 
%\[
%Y_{ijk}=\max(0,X_{ijk}).
%\]

\subsection*{Pooling}
Pooling is a downsampling of
the image, in order to reduce computational efforts and also allow
the model to be spatially invariant. The most common is \emph{max-pooling}
with kernel size $2$ and stride $2$. This replaces each 2x2 patch
in the input with its max value:
\[
Y_{ijk}=\max_{p,q\in\{0,1\}^{2}}\left[X_{2\cdot i+p,2\cdot j+q,k}\right]
\]
For general kernel size $s_{k}$ and stride $s_{s}$, we have
\[
Y_{ijk}=\max_{p,q\in\{0,\dots,s_{k}\}^{2}}\left[X_{s_{s}\cdot i+p,s_{s}\cdot j+q,k}\right]
\]
Average pooling, where the $\max$ is replaced the average, is also common.

The convolution and pooling operations generalize to 3D images in a straight-forward manner; in those cases, the input will be a stack of 3D images.


\iffalse
\begin{enumerate}
\item \emph{Softmax:} A transformation that normalizes the input across
the classes so that the output corresponds to a probability that each
pixel belongs to a certain class.
\[
P_{ijk}=\frac{\exp(X_{ijk})}{{\displaystyle \sum_{r=1}^{D_{in}}}\exp(X_{ijr})}
\]
Here $P_{ijk}$ is the probability that pixel $X_{ij}$ belongs to
class $k$.


\item \emph{Fully Connected}: Each output node of a fully connected layer
is simply an affine transformation of all nodes in the previous layer.
Let $D_{out}$ be the desired number of output nodes. Then $Y\in\mathbb{R}^{D_{out}}$
where each entry
\[
Y_{k}=W_{0}^{k}+\sum_{r=1}^{D_{in}}\sum_{q=1}^{N_{in}}\sum_{p=1}^{M_{in}}W_{pqr}^{k}X_{pqr}
\]
\item \emph{Cross-Entropy Loss}: Let $L_{ij}\in\{0,\dots,C_{out}\}$ be
the true label of pixel $X_{ij}$. The cross-entropy loss is defined
as 
\[
-\sum_{ijk}{\bf 1}_{L_{ij}=k}\log(P_{ijk})
\]
where $\mathbf{1}$ is the indicator function.
\end{enumerate}
\fi


\section*{Approximation theory}

We review some literature relating to the capabilities of neural networks
in approximating certain classes of functions. The term \emph{hidden layer(s)} is
used to refer to the intermediate layer(s) of a neural network.
The number of \emph{hidden units} refers to the dimension of the intermediate layers.

\subsection*{Universality}
Define a sigmoidal function $\sigma$ as any function with the properties:
$\lim_{x\to-\infty}\sigma(x)=0$ and $\lim_{x\to\infty}\sigma(x)=1$.
Cybenko \cite{cybenko1989approximation} showed that
neural networks with one hidden layer and an arbitrary
continuous sigmoidal function can approximate continuous functions
$f:[0,1]^d \to \mathbb{R}$ to arbitrary precision.
More precisely, let the neural network be a sum of the form
$$
f_\theta(x)= \sum_{j=1}^n c_j \sigma(W_j^T x + b_j).
$$
%are dense in $C([0,1]^d)$. 
Then, given any $f\in C([0,1]^d)$ and $\varepsilon>0$, there
exists $f_\theta$ such that
$$
|f_\theta(x)-f(x)|< \varepsilon \text{ for all } x\in [0,1]^d.
$$


%provided that no constraints are placed on the number of nodes or the size of the weights.''
% Approximation by superpositions of a sigmoidal function, by George
%Cybenko (1989) 
% Hidden layer as a basis
%\[
%B=\{\sigma(w^{\perp}x+b):w\in\mathbb{R}^{n},b\in\mathbb{R}\}.
%\]
%
% Show $\overline{\text{span}(B)}=C([0,1]^{n}).$
% The paper used the Hahn-Banach theorem, the Riesz Representation theorem,
%and some Fourier analysis.


Similarly, Hornik et. al. \cite{hornik1989multilayer} showed that a neural network, with
as few as a single hidden layer, using an arbitrary nondecreasing sigmoidal function,
is capable of approximating any Borel measurable function
$f:\mathbb{R}^d\to\mathbb{R}^m$ to any level of accuracy. 
The work of \cite{zhou2020universality} generalizes these ideas to convolutional neural networks.



%"The standard multilayer feedforward networks with as few as one hidden layer
%using arbitrary squashing functions are capable of approximating any Borel
%measurable function from one finite dimensional space to another to any desired
%degree of accuracy, provided that sufficiently many hidden units are
%available."



%\begin{itemize}
%\item 
%This paper consider a more general class of neural networks which
%form an algebra: 
%\[
%\Sigma\Pi(\sigma)=\{\sum_{j=1}^{q}\beta_{j}\cdot\Pi_{k=1}^{\ell_{j}}\sigma(A_{jk}(x)),q=1,2,\cdots\}.
%\]
%Then applies the Stone-Weierstrass theorem.
%\item The activation functions considered are ...
%\item The type of neural networks, $\Sigma(\sigma)$ networks, that we have
%been discussing correponds to $\ell_{j}\equiv1$.
%\item The passage of the universality of $\Sigma\Pi$ to $\Sigma$ goes:
%%\begin{itemize}
%%\item The universality of $\Sigma\Pi$ using the cosine activation function
%%holds. And functions in $\Sigma\Pi(\cos)$ are polynomials in cosines
%%\item Polynomials in cosines can be reduced to monomials of cosines via
%%trigonometric identities
%%\item Linear combination of cosines can be approximated to arbitrary accuracy
%%by functions in $\Sigma(\sigma)$ for any squashing function $\sigma$.
%%\end{itemize}
%\end{itemize}




%A typical statement would be as follows: Let $\mathcal{N}$
%denote a class of neural networks (e.g. convolutional neural networks),
%and $X$ a function space (e.g. $C([0,1]^{d}$). For any $0<\epsilon\le\epsilon_{0}$,
%$f\in X,$
%\[
%\exists f_{\theta}\in\mathcal{N}\,\,\,\,\text{such that }|f_{\theta}(x)-f(x)|\le\epsilon\,\,\,\forall x\in[0,1]^{d}.
%\]

%``There exist neural networks with a single hidden layer that
%approximate the given continuous function to any desired precision''.

%One immediate question is whether the space of functions that are defined by a
%network architecture is dense in the function space of interest.
%We first discuss approximation theory of neural network with a single
%hidden layer. 


%\begin{theorem}
%(Stone-Weierstrass) $A\subset\mathbb{R}^{d}$ compact, $B\subset\mathcal{C}(A,\mathbb{R}^{m}).$
%If $B$ is an algebra which separates points\emph{ and if the constant
%functions are included in $B,$ then $B$ is dense. }
%\end{theorem}


\subsection*{Rate of convergence}
However, the existence of a neural network that approximates a desired
function well does not mean that there is a good way to constructing such a
neural network, nor does it mean that the amount of computational resources
needed for its construction is acceptable.  The number of hidden units must be
sufficiently large.  A relevant question is how the number of hidden units $n$
should be increased in order meet the accuracy $\varepsilon$
and how it depends the input dimension $d$, the output dimension
$m$, and the number of training samples $N$. 

%Let $n_{\theta}$ denotes the number of neurons in network. A relevant
%question is how this number should be increased in order for the neural
%network to meet the accuracy $\epsilon$. One should also consider how
%that number depends the input dimension $d$, the output dimension
%$m$, and the number of training samples $M$. 
%\[
%n_{\theta}=n_{\theta}(d,m,M,\epsilon).
%\]







Barron \cite{barron1993universal,barron1994approximation} gives
such an analysis for a single hidden layer neural network approximating
a class of functions $f:\mathbb{R}^d \to \mathbb{R}$ with bounded domains.
The analysis also depends on the first absolute moment of the Fourier transform of $f$:
$$C_{f,d}:=\int_{\mathbb{R}^{d}}|\omega|_{1}|\hat{f}(\omega)|d\omega.$$

They use a slightly different sigmoidal function $\sigma$ which is Lipschitz and 
satisfies $\sigma(x)\rightarrow\pm1$ at least polynomially fast as $x\rightarrow\pm\infty$,
i.e., there exists $p>0$ such that $\frac{\pm1-\sigma(x)}{|x|^{p}}$ is bounded
as $x\to\pm\infty$.
The result is as follows. Define the neural network
\[
f_{\theta}(x):=\sum_{k=1}^{n}c_{k}\phi(W_{k}^T x+b_{k})+c_{0}.
\]

Then as $n,d,N\rightarrow\infty$, we have
\[
%||f-f_{\theta}||_{L^{2}([-1,1]^{2})}^{2}\sim\mathcal{O}\Big(\frac{C_{f,d}^{2}}{n}\Big)+\mathcal{O}\Big(\frac{nd}{N}\log N\Big).
||f-f_{\theta}||_2^{2}\sim\mathcal{O}\Big(\frac{C_{f,d}^{2}}{n}\Big)+\mathcal{O}\Big(\frac{nd}{N}\log N\Big).
\]

%In particular, the first and the second term on the right hand side respectively
%decreases and increases as $n$ increases (\emph{yes, the error increases
%as the number of nodes increases!} \emph{Unless the number of training
%examples also increases accordingly}), so the optimal error 

In particular, the second term on the right hand side increases as $n$ increases.
This says that increasing the network capacity (number of hidden units) leads
to \emph{overfitting} if the number of training examples does not increase accordingly.
Meanwhile, the first term decreases as $n$ increases. When 
\[
n\sim C_{f,d}\left(\frac{N}{d\log N}\right)^{1/2},
\]
the optimal error is achieved:
\[
||f-\ensuremath{f_{\theta}}|\ensuremath{|_2^{2}}\ensuremath{\ensuremath{\sim\mathcal{O}}\Big(\ensuremath{C_{f,d}\left(\frac{d}{N}\log N\right)^{1/2}}\Big)}
\]

That is, the rate of convergence relative to the number of training examples is
$\sqrt{\log N/N}$, with a rate $1/2$ that is independent of $d$. However, the
constant $C_{f,d}$ may be exponential in $d$.


%\item Summary of technical detail:
%\begin{itemize}
%\item Think of the data $(x,f(x)+\text{noise})$ being sampled by independently
%drawing $x$ from the probability distribution $\mu$ defined over
%$[-1,1]^{2}.$
%\item Estimate the optimal approximation errors in $L^{2}$ weighted by
%the probability measure $\mu$: 
%\[
%||f-f_{n,\theta^{*}}||^{2}:=\int_{[-1,1]^{2}}|f(x)-f_{n,\theta^{*}}(x)|^{2}d\mu(x)
%\]
%\item Generalization error (statistical risk): 
%\[
%||f-f_{n,\theta}||\le\underbrace{||f-f_{n,\theta^{*}}||}_{\text{approximation error}}+\underbrace{||f_{n,\theta^{*}}-f_{n,\theta}||}_{\text{estimation error}},
%\]
% where $f_{n,\theta}$ is estimated from the data with $n$ trainable
%parameters (i.e. the one found by SGD with the given data). 
%\end{itemize}

%\paragraph*{In Mhaskar's 1996 paper \cite{mhaskar1996neural}: }
%\begin{itemize}
%\item The activation function: $\sigma$ is \emph{non-polynomial} and infinitely
%differentiable. \textbf{\emph{This considtion is needed to express
%monomials by functions of the derivatives of the activation function.
%}}
%\[
%\phi_{p}(w,x):=\frac{\partial^{|p|}}{\partial w_{1}^{p_{1}}\cdots\partial w_{s}^{p_{s}}}\phi(w^{T}x+b)=x^{p}\phi^{(|p|)}(w^{T}x+b),
%\]
%\[
%x^{p}=\left(\phi^{(|p|)}(b)\right)^{-1}\phi_{p}(0;x)
%\]
% The $b$ above is a particular value at which non of the partial
%derivatives of $\phi$ vanish. This is guaranteed by the hypotheses
%on $\phi$. 
%\item Algebraic polynomials in $n$ variables of degree $<q$ are in the
%uniform closure of the span of $\mathcal{O}(q^{n})$ functions of
%the form $x\mapsto\sigma(w^{T}x+b)$.
%\item The optimal complexity of a shallow network for approximating a function
%in $W_{m}^{n}:=\{f:[-1,1]^{n}\mapsto\mathbb{R}:||f||_{\infty}+\sum_{1\le|k|\le m}||D^{k}f||\le1\}$
%to the order of $\epsilon$ point-wise is $\mathcal{O}(\epsilon^{-n/m}).$
%\end{itemize}


==> chapter-surveillance.tex <==

\begin{abstract}
We consider surveillance-evasion differential games, where a pursuer must try to constantly maintain visibility of a moving evader.  The pursuer loses as soon as the evader becomes occluded. Optimal controls for game can be formulated as a Hamilton-Jacobi-Isaac equation. We use an upwind scheme to compute the feedback value function, corresponding to the end-game time of the differential game. Although the value function enables optimal controls, it is prohibitively expensive to compute, even for a single pursuer and single evader on a small grid.  We consider a discrete variant of the surveillance-game.  We propose two locally optimal strategies based on the static value function for the surveillance-evasion game with multiple pursuers and evaders. We show that Monte Carlo tree search and self-play reinforcement learning can train a deep neural network to generate reasonable strategies for on-line game play. Given enough computational resources and offline training time, the proposed model can continue to improve its policies and efficiently scale to higher resolutions.
\end{abstract}



\section{Introduction}

We consider a multiplayer \emph{surveillance-evasion} game consisting of two
teams, the pursuers and the evaders. The pursuers must maintain line-of-sight
visibility of the evaders for as long as possible as they move through an
environment with obstacles. Meanwhile, the evaders aim to hide from the
pursuers as soon as possible. The game ends when the pursuers lose sight of the
evaders. We assume all players have perfect knowledge of the obstacles and the
game is closed-loop -- each player employs a feedback strategy, reacting
dynamically to the positions of all other players. 

%The game can be divided into two settings, open loop and closed loop.
%In closed loop, the controls are dynamic and change as the actions occur.
%In open loop, the players select their control at the beginning and cannot change the actions as the game progresses.
%These games are useful in applications such as autonomous target tracking and babysitting.
In section~\ref{sec:hji}, we consider the game in the context of Hamilton-Jacobi-Isaacs
(HJI) equations.  We propose a scheme to compute the value function, which,
informally, describes how "good" it is for each player to be in a specific
state. Then each player can pick the strategy that optimizes the value function
locally. Due to the principal of optimality, local optimization with respect to
the value function is globally optimal. This is because the value function
encodes information from all possible trajectories. As a result, the value
function is also very expensive to compute.

Section~\ref{sec:locally} discusses locally-optimal policies and
section~\ref{sec:learning-policy} presents search-based methods
to learn policies for the multiplayer version of the game.



\subsection{Related works}

The surveillance-evasion game is related to a popular class of games called
pursuit-evasion \cite{ho1965differential,isaacs1965differential}, where the
objective is for the pursuer to physically capture the evader.  Classical
problems take place in obstacle-free space with constraints on the players'
motion. Variants include the lion and man
\cite{karnad2009lion,sgall2001solution}, where both players have the same
maneuverability,  and the homicidal chauffeur \cite{merz1974homicidal}, where
one player drives a vehicle, which is faster, but has constrained mobility. 
Lewin et. al. \cite{lewin1975surveillance} considered a
game in an obstacle-free space, where the pursuer must keep the evader within a
detection circle.  


Bardi et. al. \cite{bardi1999numerical} proposed a semi-Lagrangian scheme for
approximating the value function of the pursuit-evasion game as viscosity solution
to the Hamilton-Jacobi-Isaacs equation, in a bounded domain with no obstacles.
In general, these methods are very expensive, with complexity $\bigo(m^{kd})$ where
$k$ is the number of players and $d$ is the dimension. This is because the
value function, once computed, can provide the optimal controls for all
possible player positions. 
A class of methods try
to deal with the curse of dimensionality by solving for the solutions of
Hamilton-Jacobi equations at individual points in space and time. These methods
are causality-free; the solution at one point does not depend on solutions at
other points, making them conveniently parallelizable. They are efficient,
since one only solves for the value function locally, where it is needed,
rather than globally.  Chow et. al.
\cite{chow2017algorithm,chow2018algorithm,chow2019algorithm} use the Hopf-Lax
formula to efficiently solve Hamilton-Jacobi equations for a class of
Hamiltonians.  Sparse grid characteristics, due to Kang et. al. \cite{kang2017mitigating}, is another
causality-free method which finds the solution by solving a boundary value
problem for each point.  Unfortunately, these methods do not apply to domains
with obstacles since they cannot handle boundary conditions.  

% Sparse grid characteristics method requires convexity assumptions on the Hamiltonian.  Also, they use their method to train neural network to do inference efficiently.  



The visibility-based pursuit-evasion game, introduced by Suzuki. et. al
\cite{suzuki1992searching}, is a version where the
pursuer(s) must compute the shortest path to find all hidden evaders in a
cluttered environment, or report it is not possible. The number of evaders is
unknown and their speed is unbounded.  Guibas et. al.
\cite{guibas1997visibility} proposed a graph-based method for polygonal
environments.  Other settings include multiple pursuers
\cite{stiffler2014complete}, bounded speeds \cite{tovar2008visibility},
unknown, piecewise-smooth planar environments \cite{sachs2004visibility}, and
simply-connected two-dimensional curved environments
\cite{lavalle2001visibility}.

The surveillance-evasion game has been studied previously
in the literature. 
LaValle et. al. \cite{lavalle1997motion} use dynamic programming to compute
optimal trajectories for the pursuer, assuming a known evader trajectory. For
the case of an unpredictable evader, they suggest a local heuristic: maximize
the probably of visibility of the evader at the next time step.
They also mention, but do not implement, an idea to locally maximize the evader's time to occlusion.


Bhattacharya et. al. \cite{bhattacharya2008approximation,bhattacharya2011cell}
used geometric arguments to partition the environment into several regions
based on the outcome of the game.  
%evader can successfully escape, for environments with polygonal and smooth convex obstacles.  %They do not suggest controls.
In \cite{bhattacharya2009existence,zou2018optimal}, they use geometry and optimal control to compute
optimal trajectories for a single pursuer and single evader near the corners of a polygon.
The controls are then extended to the whole domain containing polygonal obstacles by partitioning based on the corners
\cite{zou2016optimal},
for the finite-horizon tracking problem \cite{zou2016visibility},
and for multiple players by allocating a pursuer for each evader via the Hungrarian matching algorithm
\cite{zhang2016multi}.
%extends to multiple players by allocating a purser to each evader through a Hungrarian matching algorithm using a designed risk function.
%In \cite{zou2016optimal}, they consider the optimal controls around a corner, and extend to general polygonal environments by designing pursuit partions, ways to weight the strategies around each corner based on distance/time.

Takei et. al. \cite{takei2014efficient} proposed an efficient
algorithm for computing the static value function corresponding to the open loop game,
where each player moves according to a fixed strategy determined at initial time.
Their open loop game is conservative towards the pursuer, since the evader can
optimally counter any of the pursuer's strategies. As a consequence, the game
is guaranteed to end in finite time, as long as the domain is not
star-shaped. %The computational cost is $\bigo(m^{2d})$ in $d$ dimensions, where $m$ is the size of the grid in one dimension.  The algorithm is parallelizable.
In contrast, a closed loop game allows players to react dynamically to each other's actions.

In \cite{cartee2019time,gilles2019evasive,takei2015optimal}, the authors
propose optimal paths for an evader to reach a target destination, while
minimizing exposure to an observer.  In \cite{gilles2019evasive}, the observer
is stationary.  In \cite{cartee2019time}, the observer moves according to a
fixed trajectory.  In \cite{takei2015optimal}, the evader can tolerate brief
moments of exposure so long as the consecutive exposure time does not exceed a
given threshold.  In all three cases, the observer's controls are restricted to
choosing from a known distribution of trajectories; they are not allowed to
move freely.% within the domain.

Bharadwaj et. al. \cite{bharadwaj2018synthesis} use reactive synthesis to
determine the pursuer's controls for the surveillance-evasion game on a discrete
grid. They propose a method of \emph{belief abstraction} to coarsen the state
space and only refine as needed.  The method is quadratic in the number of
states: $\bigo(m^{2kd})$ for $k$ players.  While it is more computationally
expensive than the Hamilton-Jacobi based methods, it is more flexible in being
able to handle a wider class of temporal surveillance objectives, such as
maintaining visibility at all times, maintaining a bound on the spatial
uncertainty of the evader, or guaranteeing visibility of the evader infinitely
often.

Recently, Silver et. al developed the AlphaGoZero and AlphaZero programs that
excel at playing Go, Chess, and Shogi, without using any prior knowledge of the
games besides the rules \cite{silver2017mastering,silver2017mastering2}. They
use Monte Carlo tree search, deep neural networks and self-play reinforcement
learning to become competitive with the world's top professional players.

%Inspired by their work, we apply Monte Carlo tree search and self-play reinforcement learning to the surveillance-evasion games.
%These games are symmetric, since the goals of the players are identical. 
%In our games, the goals for the pursuer and evader differ.

\subsection*{Contributions}
We use a Godunov upwind scheme to compute the value function for the
closed loop surveillance-evasion game with obstacles in two dimensions.  The
state space is four dimensional.  The value function allows us to compute the
optimal feedback controls for the pursuers and evaders. Unlike the static game
\cite{takei2014efficient}, it is possible for the pursuer to win. However, the
computation is $\bigo(m^{kd})$ where $k$ is the number of players and $d$ the
dimensions.

As the number of players grows, computing the value function becomes infeasible.
We propose locally optimal strategies for the multiplayer surveillance-evasion
game, based on the value function for the static game.  In addition, we propose
a deep neural network trained via self play and Monte Carlo tree search to
learn controls for the pursuer.  Unlike Go, Chess, and Shogi, the
surveillance-evasion game is not symmetric; the pursuers and evaders require
different tactics. We use the local strategies to help improve the
efficiency of self-play.

The neural network is trained offline on a class of environments.  Then,
during play time, the trained network can be used to play games efficiently on
previously unseen environments.  That is, at the expense of preprocessing time
and optimality, we present an algorithm which can run efficiently. While the
deviation from optimality may sound undesirable, it actually is reasonable.
Optimality assumes perfect actions and instant reactions.  It real
applications, noise and delays will perturb the system away from optimal
trajectories.  We show promising examples in 2D.  

%Lastly, we show application 
%surveillance-constrained visibility optimization problem.  There, in addition
%to a strict surveillance requirement, the agent must continually patrol the
%environment.


\section{Value function from HJI equation}
\label{sec:hji}

Without loss of generality, we formulate the two player game, with a single pursuer and single evader.
The domain $\domain\subseteq \mathbb{R}^d$ consists of obstacles and free space:
$\domain=\obs\cup\free$.  Consider a pursuer and evader whose positions at a particular time instance
are given by $\xp,\xe:[0,\infty) \to \free$, respectively. 
Let $A:= S^{d-1}\cup \{{\bf 0}\}$ be the compact set of control values.
The feedback controls map the players' positions to a control value:
\beq\pcontrol,\econtrol\in\admiss:=\{\sigma:\free\times\free\to A \ | \ \sigma \text{ measurable}\},\eeq
where $\admiss$ is the set of admissible controls.
The players move with velocities $\pspeed,\espeed:
\domain \to [0,\infty)$ according to the dynamics

\beq
%\dot{\xp}(t) &= \pspeed(\xp(t)) \pcontrol(\xp(t),\xe(t))  \qquad &\dot{\xe}(t) &= \espeed(\xe(t)) \econtrol(\xp(t),\xe(t))\\
\dot{\xp}(t) &= \pspeed(\xp(t)) \pcontrol(\xp(t),\xe(t))  \qquad &\dot{\xe}(t) &= \espeed(\xe(t)) \econtrol(\xp(t),\xe(t))\\
\xp(0)&= \xpinit \qquad &\xe(0)&= \xeinit \\
\eeq


%Notice the controls dynamically respond to the current positions for each player. 
For clarity of notation, we will omit the dependence of the controls on
the players' positions.  For simplicity, we assume velocities are isotropic,
meaning they do not depend on the controls. In real-world scenarios, this may not
be the case.  For example, an airplane's dynamics might be constrained by its
momentum and turning radius.

As a slight relaxation, we consider the finite-horizon version of the game, where the pursuers
win if they can prolong the game past a time threshold $T$.
Let $\failset := \{(\xp(\cdot),\xe(\cdot)) | \shadow(\xp(\cdot),\xe(\cdot))\le 0\}$ be the end-game set of losing positions,
where $\shadow$ is the shadow function defined in section~\ref{sec:shadow}.
Define the payoff function 
\beq 
\cost[\xpinit,\xeinit,t,\pcontrol,\econtrol] :=
\inf\{0\le \tau \le t|(\xp(\tau),\xe(\tau)) \in \failset \},
\eeq
where $\cost[\xpinit,\xeinit,t,\pcontrol,\econtrol]:=t$ if the set $(\xp(\tau),\xe(\tau))\in\failset$ is empty.
The payoff is the minimum time-to-occlusion for given set
initial positions and controls.
Define the finite-horizon value function as:
\beq
\val(\xpinit,\xeinit,t) = \sup_{\pcontrol\in\admiss} \inf_{\econtrol\in\admiss} \cost[\xpinit,\xeinit,t,\pcontrol,\econtrol] 
\eeq

The value function describes the length of the game played to time $t$, starting from all pairs of initial positions, and assuming optimal controls.
We are interested in $\val(\xpinit,\xeinit,T)$ for a sufficiently large $T$, which characterizes
the set of initial positions from which the pursuers can maintain visibility of the evaders
for at least $T$ time units.
As $T\to \infty$, we recover the infinite-horizon value function.

By using the principle of optimality and Taylor expansion, one can derive
the Hamilton-Jacobi-Isaacs equation \cite{bardi2008optimal,crandall1983viscosity,evans1984differential}:
\iffalse
Consider a pair of initial positions $\xpinit$ and $\xeinit$. For clarify of notation, we use $\xp(t)$ and $\xe(t)$ to denote the positions
of the pursuer and evader at time $t$ according to the controls $\pcontrol$ and $\econtrol$, assuming $\xp(0)=\xpinit$ and $\xe(0)=\xeinit$.
The value function satisfies the Dynamic Programming Principle:
\begin{align}
\val(\xpinit,\xeinit) &= \sup_\pcontrol \inf_\econtrol \cost[\xpinit,\xeinit,\pcontrol,\econtrol]  \\
&= t + \sup_\pcontrol \inf_\econtrol   \cost[\xp(t),\xe(t),\pcontrol,\econtrol]  \\
&=   t + \sup_\pcontrol \inf_\econtrol  \val(\xp(t),\xe(t) ) 
\end{align}



Rearranging and dividing by $t>0$, we have
\beq
%\val(\xpinit,\xeinit) -  \val(\xp(t),\xe(t)) &= t \\
\frac{1}{t} \Big[ \val(\xpinit,\xeinit) -  \val(\xp(t),\xe(t))\Big]  &= 1 
\label{eq:dpp}
\eeq

By Taylor expansion, we have
\begin{align}
\xp(t) &= \xpinit + t \dot{\xp}(0) + \bigo(t^2) \\
\xe(t) &= \xeinit + t \dot{\xe}(0) + \bigo(t^2) \\ 
%\val(\xp(t),\xe(t)) &= \val(\xpinit,\xeinit) + \nabla_\xp \val \big(\xp(t)-\xpinit\big) + \nabla_\xe \val \big(\xe(t)-\xeinit\big) + \bigo(t^2)\\
\val(\xp(t),\xe(t)) &= \val(\xpinit,\xeinit) + t \ \nabla_\xp \val \cdot \dot{\xp}(0) + t \ \nabla_\xe \val \cdot \dot{\xe}(0) + \bigo(t^2)
\end{align}

Substituting back into (\ref{eq:dpp}), and taking the limit
\begin{align}
\lim_{t\to0^+} \frac{1}{t} \Big[ \val(\xpinit,\xeinit) -  \val(\xp(t),\xe(t))\Big]  &= 1 \\
\lim_{t\to0^+} \frac{1}{t} \Big[ -t \ \nabla_\xp \val \cdot \dot{\xp}(0) - t \ \nabla_\xe \val \cdot \dot{\xe}(0) + \bigo(t^2) \Big] &= 1 \\
- \ \nabla_\xp \val \cdot \dot{\xp}(0) -  \ \nabla_\xe \val \cdot \dot{\xe}(0)  &= 1 \\
- \pspeed(\xpinit)\ \nabla_\xp \val \cdot  \pcontrol(\xpinit,\xeinit) -  \espeed(\xeinit) \ \nabla_\xe \val \cdot \econtrol(\xpinit,\xeinit)  &= 1
\end{align}
\fi
\beq
\val_t + \inf_{\econtrol\in A} \sup_{\pcontrol \in A} \{-\nabla_\xp \val \cdot \pcontrol - \nabla_\xe \val \cdot \econtrol\}
&= 1 \ ,  &\text{ on } \free\setminus\failset \\
\val(\xp,\xe,0) &= 0 \\
\val(\xp,\xe,t) &= 0 \ , & (\xp,\xe)\in\failset \\
\val(\xp,\xe,t) &= \infty \ , & \xp \text{ or }\xe \in \obs \label{eq:hji}
\eeq
It has been shown the value function is the viscosity solution \cite{bardi2008optimal,crandall1983viscosity,evans1984differential} to \eqref{eq:hji}.
For isotropic controls, this simplifies to the following Eikonal equation:
\beq
\val_t -\pspeed |\nabla_\xp \val| +\espeed |\nabla_\xe \val|  &= 1 \ ,  &\text{ on } \free\setminus\failset \\
\val(\xp,\xe,0) &= 0 \\
\val(\xp,\xe,t) &= 0 \ , & (\xp,\xe )\in \failset \\
\val(\xp,\xe,t) &= \infty \ , & \xp \text{ or }\xe \in \obs \label{eq:hji-eikonal}
\eeq
The optimal controls can be recovered by computing the gradient of the value function:
\begin{align} \label{eq:optcontrols}
\pcontrol &=  \frac{\nabla_\xp \val}{|\nabla_\xp \val|} \ , \qquad
\econtrol =  -\frac{\nabla_\xe \val}{|\nabla_\xe \val|} \ .
\end{align}
%Remark: note there are other variants of the value function where the limits of
%integration do not depend on the controls, such as finite-horizon or
%infinite-horizon optimal control problem.  The resulting PDE is similar, but
%perhaps without the boundary conditions.  See, for example, [CITE]. 
%\todo{Or the appendix}.
%(I could technically stick with a time dependent formulation with a large penalty, but there's no guarantee)

\subsection{Algorithm}
\iffalse
We solve (\ref{eq:hji-eikonal}) as the steady state of the time-dependent equation \cite{osher1993level}:
\beq
\val_t -\pspeed |\nabla_\xp \val| +\espeed |\nabla_\xe \val|  &= 1 \qquad &\text{ on } \free\setminus\failset \\
\val(\xp,\xe,t) &= 0 &\qquad (\xp,\xe )\in \failset \\
\val(\xp,\xe) &= \infty &\qquad \xp \text{ or }\xe \in \obs \label{eq:hji-eikonal-time}
\eeq
\fi

Following the ideas in \cite{tsai2003fast}, we discretize the gradient using upwind scheme as follows.
Let $\xp_{i,j},\xe_{k,l}\in\free$ be the discretized positions with grid
spacing $h$.  Denote $\val_{i,j,k,l}$ as the numerical solution to (\ref{eq:hji-eikonal}) for
initial positions $\xp_{i,j},\xe_{k,l}$.  We estimate the gradient using finite
difference. For clarity, we will only mark the relevant subscripts, e.g.
$\val_{i+1}:=\val_{i+1,j,k,l}$.

%\beq
%\partial_{P_x}\val &= \frac{1}{h} \max \Big( \max(\val_{i}-\val_{i-1},0), \min(\val_{i+1}-\val_{i},0) \Big), \\
%\eeq

%\beq
%\xp_{x-} &= \frac{1}{h} \Big(\val_{i,j,k,l} - \val_{i-1,j,k,l}\Big), \qquad  &\xe_{x-} = \frac{1}{h} \Big(\val_{i,j,k,l} - \val_{i,j,k-1,l}\Big),\\
%\xp_{x+} &= \frac{1}{h} \Big(\val_{i+1,j,k,l} - \val_{i,j,k,l}\Big), \qquad  &\xe_{x+} = \frac{1}{h} \Big(\val_{i,j,k+1,l} - \val_{i,j,k,l}\Big),\\
%\xp_{y-} &= \frac{1}{h} \Big(\val_{i,j,k,l} - \val_{i,j-1,k,l}\Big), \qquad  &\xe_{y-} = \frac{1}{h} \Big(\val_{i,j,k,l} - \val_{i,j,k,l-1}\Big),\\
%\xp_{y+} &= \frac{1}{h} \Big(\val_{i,j+1,k,l} - \val_{i,j,k,l}\Big), \qquad  &\xe_{y+} = \frac{1}{h} \Big(\val_{i,j,k,l+1} - \val_{i,j,k,l}\Big).
%\eeq

%\beq
%\xp_{-}^x &= \frac{1}{h} \Big(\val_{i} - \val_{i-1}\Big), \qquad  &\xe_{-}^x &= \frac{1}{h} \Big(\val_{k} - \val_{k-1}\Big),\\
%\xp_{+}^x &= \frac{1}{h} \Big(\val_{i+1} - \val_{i}\Big), \qquad  &\xe_{+}^x &= \frac{1}{h} \Big(\val_{k+1} - \val_{k}\Big),\\
%\xp_{-}^y &= \frac{1}{h} \Big(\val_{j} - \val_{j-1}\Big), \qquad  &\xe_{-}^y &= \frac{1}{h} \Big(\val_{l} - \val_{l-1}\Big),\\
%\xp_{+}^y &= \frac{1}{h} \Big(\val_{j+1} - \val_{j}\Big), \qquad  &\xe_{+}^y &= \frac{1}{h} \Big(\val_{l+1} - \val_{l}\Big).
%\eeq

\beq
\xp_{x^-} &:= \frac{1}{h} \Big(\val_{i} - \val_{i-1}\Big), \qquad  &\xe_{x^-} &:= \frac{1}{h} \Big(\val_{k} - \val_{k-1}\Big),\\
\xp_{x^+} &:= \frac{1}{h} \Big(\val_{i+1} - \val_{i}\Big), \qquad  &\xe_{x^+} &:= \frac{1}{h} \Big(\val_{k+1} - \val_{k}\Big),\\
\xp_{y^-} &:= \frac{1}{h} \Big(\val_{j} - \val_{j-1}\Big), \qquad  &\xe_{y^-} &:= \frac{1}{h} \Big(\val_{l} - \val_{l-1}\Big),\\
\xp_{y^+} &:= \frac{1}{h} \Big(\val_{j+1} - \val_{j}\Big), \qquad  &\xe_{y^+} &:= \frac{1}{h} \Big(\val_{l+1} - \val_{l}\Big).\\
\eeq

Let $a^- := -\min(0,a)$ and
$a^+ := \max(0,a)$. Define
\beq
\sgn\max(a,b) &:= 
\begin{cases}
a^+ & \text{ if } \max(a^+,b^-) = a^+ \\
-b^- & \text{ if } \max(a^+,b^-) = b^- \\
\end{cases} \\
\eeq

and

\beq
\partial \xp_x \val &= \sgn\max (\xp_{x^+}, \xp_{x^-} ) \\
\partial \xp_y \val &= \sgn\max (\xp_{y^+}, \xp_{y^-} ) \\
\partial \xe_x \val &= \sgn\max (\xe_{x^-}, \xe_{x^+} ) \\
\partial \xe_y \val &= \sgn\max (\xe_{y^-}, \xe_{y^+} ) \\
\eeq

Finally, the desired numerical gradients are
\beq
|\nabla_\xp \val| &= \Big( (\partial \xp_x \val )^2 + (\partial \xp_y \val)^2 \Big)^{1/2} \\
|\nabla_\xe \val| &= \Big( (\partial \xe_x \val )^2 + (\partial \xe_y \val)^2 \Big)^{1/2} \\
\eeq

Then we have a simple explicit scheme.
\beq
\val^{n+1} = \val^{n} + \Delta t (1 + \pspeed |\nabla_\xp \val| - \espeed |\nabla_\xe \val| ) 
\label{eq:hji-scheme}
\eeq
The CFL conditions dictate that the time step $\Delta t$ should be
\beq
\Delta t \le \frac{h}{16 \max(\pspeed,\espeed)}
\eeq

For a given environment, we precompute the value function by iteration until convergence.
During play time, we initialize $\xpinit,\xeinit$ and compute the optimal trajectories according to
(\ref{eq:optcontrols}) using $\Delta t$ time increments.

\subsubsection{Boundary conditions}
The obstacles appear in the HJI equation as boundary conditions.
However, direct numerical implementation leads to artifacts near the obstacles.
Instead, we model the obstacles by setting the velocities to be small inside obstacles.
We regularize the velocities by adding a smooth transition \cite{takei2014efficient}:

\begin{align}
v_\epsilon(x) &=
\begin{cases}
v(x) & \map(x)>0 \\
v_\text{min} + \frac{v(x)-v_\text{min}}{2} \Big[ \cos\Big(\frac{\phi(x)\pi}{2\epsilon}\Big)+1 \Big]  & \map(x)\in[-2\epsilon,0]\\
v_\text{min} & \map(x) < -2\epsilon
\end{cases}
\end{align}
where $\map$ is the signed distance function to the obstacle boundaries.
In the numerical experiments, we use $\epsilon=16\Delta x$ and $v_\text{min} = 1/100$.

\subsection{Numerical results}


\subsubsection*{Stationary pursuer}
We verify that the scheme converges numerically for the case in which the pursuer is stationary. 
When $\pspeed=0$, the HJI equation \eqref{eq:hji-eikonal} becomes the time-dependent Eikonal equation:
\beq
\val_t + \espeed |\nabla_\xe \val|  &= 1 \qquad &\text{ on } \free\setminus\failset \\
\val(\xp,\xe,0) &= 0 \\
\val(\xp,\xe,t) &= 0 &\qquad (\xp,\xe )\in \failset \label{eq:hji-stationary}
\eeq
In particular, for sufficiently large $t$, the value function reaches a steady state, and satisfies the Eikonal equation:
\beq
\espeed |\nabla_\xe \val|  &= 1 \qquad &\text{ on } \free\setminus\failset \\
\val(\xp,\xe) &= 0 &\qquad (\xp,\xe )\in \failset \label{eq:hji-stationary-steady}
\eeq
For this special case, the exact solution is known; the solution corresponds to the evader's travel time to
the end-game set $\failset$.
Also, this case effectively reduces the computational cost
from $\bigo(m^4)$ to $\bigo(m^2)$, so that we can reasonably compute solutions at higher resolutions.

We consider a $\domain=[0,1)\times[0,1)$ with a single circular obstacle of radius $0.15$ centered at $(1/2,1/2)$.
The pursuer is stationary at $\xp_0=(1/8,1/2)$. 
We use $\Delta t = \Delta x/20$ and iterate until the solution no longer changes in the $L_1$ sense, using a tolerance of $10^{-5}$.

We compute the ``exact'' solution using fast marching method on high resolution grid $M=2048$.
We vary $m$ from $16$ to $1024$ and observe convergence in the $L_1$ and $L_2$ sense,
as seen in Table~\ref{tab:hji_conv}.
In Figure~\ref{fig:hji_contour}, we plot the level curves comparing the computed solution at $m=512,1024$ to the ``exact'' solution.
Notice the discrepancies are a result of the difficulty in dealing with boundary conditions.
However, these errors decay as the grid is refined.

The case where the evader is stationary is not interesting.

\begin{table}[]
\begin{center}
\caption{Error for the stationary pursuer case, compared to the known solution computed using fast marching method at resolution $M=2048$.\vspace{1em}}
\label{tab:hji_conv}

\begin{tabular}{c|c|c}
$m   $ & $L_1$ error             & $L_2$ error            \\ 
\hline
$16  $ & $0.08972215 $ &$0.01288563 $ \\
$32  $ & $0.03177683 $ &$0.00159669 $ \\
$64  $ & $0.02442984 $ &$0.00111537 $ \\
$128 $ & $0.01059728 $ &$0.00021345 $ \\
$256 $ & $0.00515584 $ &$0.00005214 $ \\
$512 $ & $0.00304322 $ &$0.00001961 $ \\
$1024$ & $0.00086068 $ &$0.00000142 $
\end{tabular}
\end{center}
\end{table}



%$16  $ & $0.08972215762198651  $ &$0.012885633288809298 $ \\
%$32  $ & $0.031776830083754815 $ &$0.001596690139730697 $ \\
%$64  $ & $0.024429847742256806 $ &$0.001115370592972781 $ \\
%$128 $ & $0.010597284307555795 $ &$0.000213453745010690 $ \\
%$256 $ & $0.005155845526871389 $ &$0.000052147495364447 $ \\
%$512 $ & $0.003043227116595554 $ &$0.000019619974499759 $ \\
%$1024$ & $0.000860688403850700 $ &$0.000001424361236251 $


   \begin{figure}[hptb]
      \centering
      \includegraphics[width=.45\textwidth]{figures/hj_convergence_512.pdf} \quad
      \includegraphics[width=.45\textwidth]{figures/hj_convergence_1024.pdf}

	  \caption{Comparison of contours of the ``exact'' solution (blue) with those
computed by the scheme (\ref{eq:hji-scheme}) (red) using grid resolutions $m=512$ (left) and
$m=1024$ (right).  The pursuer (blue square) is stationary.  The error emanates from the obstacle
due to boundary conditions, but the scheme converges
as the grid is refined.} \label{fig:hji_contour}

\end{figure}



\subsubsection*{A circular obstacle}

The evader has the advantage in the surveillance-evasion game. It is
difficult for the pursuer to win unless it is sufficiently fast.
But once it is fast enough, it can almost always win. 
Define the winning regions for the pursuer and evader, respectively:
\begin{align}
\mathcal{W}_\xp &= \{(\xp,\xe) | \val(\xp,\xe) > T_\text{max}\} \\
\mathcal{W}_\xe &= \{(\xp,\xe) | \val(\xp,\xe) \le T_\text{max}\} 
\end{align}

Here, we use $T_\text{max}=.9 T$ to tolerate numerical artifacts due to boundary conditions.  
In Figure~\ref{fig:hj_circles_winset}, we show how the winning region
for a fixed evader/pursuer position changes as the pursuer's speed increases.
Since it is difficult to visualize data in
4D, we plot the slices $\val(\xpinit,\cdot)$ and $\val(\cdot,\xeinit)$ where
$\xpinit=\xeinit=(1/8,1/2)$. 
We use $m=64$, $\Delta t = \Delta x/20$ and iterate until $T=10$.
We fix $\pspeed=1$ and compute $\val$ for each $\espeed\in\{\frac{1}{3},\frac{1}{2},\frac{2}{3}\}$.
The computation for each value function takes 16 hours.


%As P's speed increases, it becomes less necessary to move, because it can always catch up.
%Also, P can force E into a fixed point, where it becomes impossible to win. In this case,
%E becomes stationary and is essentially \emph{captured}.



   \begin{figure}[hptb]
      \centering
      %\includegraphics[width=.78\textwidth]{figures/hj_circle_winsets_cE_100.pdf} 
      \includegraphics[width=.78\textwidth]{figures/hj_circle_winsets_cE_66.pdf}
      \includegraphics[width=.78\textwidth]{figures/hj_circle_winsets_cE_50.pdf}
      \includegraphics[width=.78\textwidth]{figures/hj_circle_winsets_cE_33.pdf}
	  \caption{Comparison of winning initial positions for the evader (left,
red contour) against a pursuer with fixed initial position (blue square) and
vice versa -- winning initial positions for the pursuer (right, blue contour)
against an evader with fixed initial position (red circle).  Left column shows
$\val(\xpinit,\cdot)$ while right column shows $\val(\cdot,\xeinit)$, where higher values of
$\val$ are yellow, while lower values are dark blue. From top to bottom, the pursuer is $1.5$, $2$
and $3$ times faster than the evader.  
The pursuer must be sufficiently fast to have a chance at winning.
} \label{fig:hj_circles_winset} \end{figure}



Figure~\ref{fig:hj_circles_traj} shows trajectories from several initial positions
with various speeds. Interestingly, once the evader is cornered, the optimal controls
dictate that it is futile to move. That is, the value function is locally constant.


   \begin{figure}[hptb]
      \centering
      \includegraphics[width=.45\textwidth]{figures/hj_traj_circles_32_08_04_60_cE_100.pdf}
      %\includegraphics[width=.45\textwidth]{figures/hj_traj_circles_32_08_04_60_cE_66.pdf}
      \includegraphics[width=.45\textwidth]{figures/hj_traj_circles_32_08_04_60_cE_50.pdf}
      %\includegraphics[width=.45\textwidth]{figures/hj_traj_circles_32_08_04_60_cE_33.pdf}
      %\includegraphics[width=.45\textwidth]{figures/hj_traj_circles_16_08_04_60_cE_100.pdf}
      %\includegraphics[width=.45\textwidth]{figures/hj_traj_circles_16_08_04_60_cE_66.pdf}
      %\includegraphics[width=.45\textwidth]{figures/hj_traj_circles_16_08_04_60_cE_50.pdf}
      %\includegraphics[width=.45\textwidth]{figures/hj_traj_circles_16_08_04_60_cE_33.pdf}
      \includegraphics[width=.45\textwidth]{figures/hj_traj_circles_48_08_04_32_cE_100.pdf}
      %\includegraphics[width=.45\textwidth]{figures/hj_traj_circles_48_08_04_32_cE_66.pdf}
      \includegraphics[width=.45\textwidth]{figures/hj_traj_circles_48_08_04_32_cE_50.pdf}
      %\includegraphics[width=.45\textwidth]{figures/hj_traj_circles_48_08_04_32_cE_33.pdf}

	  \caption{Trajectories of several games played around a circle. The
pursuer loses when it has same speed as the evader (left column). When the pursuer is 2x faster than the evader,
it is possible to win; the evader essentially gives up once it is cornered, since no controls will change the outcome (right column).
Initial positions are shown as stars. Black lines connect positions at constant time intervals.}

\label{fig:hj_circles_traj} \end{figure}


\subsubsection*{More obstacles}
In Figure~\ref{fig:hj_dice_traj} we consider a more complicated environment with multiple obstacles.
Here, the pursuer is twice as fast as the evader. Although there are many obstacles, the dynamics
are not so interesting in the sense that the evader will generally navigate towards a single obstacle.
Again, the evader tends to give up once the game has been decided.

Finally, in Figure~\ref{fig:hj_human_traj} we show suboptimal controls for the
evader. In particular, the evader is controlled manually. Although manual
controls do not help the evader win, they lead to more interesting
trajectories.

   \begin{figure}[htb]
      \centering
      \includegraphics[width=.45\textwidth]{figures/hj_traj_dice_32_08_07_37_cE_50.pdf}
      \includegraphics[width=.45\textwidth]{figures/hj_traj_dice_56_08_57_35_cE_50.pdf}
	  \caption{Trajectories of games played around 5 circular obstacles. Pursuer (blue) is 2x as fast as evader (red).
The evader wins (left) if it can quickly hide. Otherwise it will give up once it is captured (right).
Initial positions are shown as stars. Black lines connect positions at constant time intervals.}
\label{fig:hj_dice_traj} \end{figure}
   \begin{figure}[hptb]
      \centering
      \includegraphics[width=.45\textwidth]{figures/hj_traj_circles_32_08_32_21_cE_33_human.pdf}
      \includegraphics[width=.45\textwidth]{figures/hj_traj_dice_56_08_57_35_cE_50_human.pdf}
	  \caption{Manually controlled evader against an optimal pursuer. The evader loses in both cases, but does not give up.}
\label{fig:hj_human_traj} \end{figure}




\subsection{Discussion}
Notice that an optimal trajectory for the pursuer balances distance and
visibility.  While moving closer to the evader will guarantee that it can't
``get away'', it is not sufficient, since being close leads to more
occlussions. On the other hand, moving far away gives better visibility of the
environment, but may make it impossible to catch up once E turns the corner.

Although we described the formulation for a single pursuer and evader,
the same scheme holds for multiple pursuers and evaders. The end-game set just
needs to be modified to take into account the multiple players.
That is, the game ends as soon as any evader is occluded from all pursuers.
However, the computational complexity of the scheme is $\bigo(m^{kd})$ which
quickly becomes unfeasible even on small grid sizes.
At the expense of offline compute time, the game can be played efficiently
online. The caveat is that, the value function is only valid for the specific
map and velocities computed offline.

%Note that in the limit of infinite evaders, the game reduces to the surveillance problem from chapter~\ref{chap:exploration}.





\section{Locally optimal strategies}
\label{sec:locally}
%Given enough MCTS iterations and training time, one can expect
%that the neural network trained using self play can continue to improve.
%However, it may only be feasible for large research labs which have access to
%vast computational resources.
%One may consider strategies to help improve the efficiency of
%self-play. 
%Or one may want to train a better evader.
%This can be done using, for example, the pursuer's neural network.

As the number of players increases, computing the value function from the HJI
equations is no longer tractable.
We consider a discrete version of the game, with the aim of feasibly
computing controls for games with multiple pursuers and multiple evaders.  
Each player's position is now restricted on a grid, and at each turn,
the player can move to a new position within a neighborhood determined by its
velocity. Players cannot move through obstacles. 
Formally, define the arrival time function
\beq
\parrival(x,y) &:= \min_{\pcontrol\in\admiss} \min \{t|\xp(0)=x,\xp(t)=y\}\\
\earrival(x,y) &:= \min_{\econtrol\in\admiss} \min \{t|\xe(0)=x,\xe(t)=y\}  .
\eeq
The set of valid actions are the positions $y$ which can be reached from $x$
within a $\Delta t$ time increment:
\beq
\pvalid(t)&:=\{y\in\free | \parrival(\xp(t),y) \le \Delta t\}\\
\evalid(t)&:=\{y\in\free | \earrival(\xe(t),y) \le \Delta t\}.
\eeq
In a $\Delta t$ time step, each player can move to a position
\beq
\xp(t+\Delta t) \in \pvalid(t) \\
\xe(t+\Delta t) \in \evalid(t).
\eeq

Analogously, for multiple players, denote the number of pursuers and evaders as
$k_P$ and $k_E$, respectively. Define
\beq
\bfxp &= (\xp_1,\dots, \xp_{k_P})\\
\bfxe &= (\xe_1,\dots, \xe_{k_E})\\
\bfpvalid(t) &= \{\bfxp| \xp_i \in \pvalid(t) \ , \ i=1,\dots,k_P\} \\
\bfevalid(t) &= \{\bfxe| \xe_j \in \evalid(t) \ , \ j=1,\dots,k_E\}
\eeq
so that in $\Delta t$ time, each team can move to
\beq
\bfxp(t+\Delta t) \in \bfpvalid(t) \\
\bfxe(t+\Delta t) \in \bfevalid(t) \\
\eeq

The game ends as soon as one evader is occluded from all
pursuers. The end-game set is
\beq
\failset = \{ (\bfxp,\bfxe) \ |\ \exists \ j : \shadow(\xp_i,\xe_j)\le 0 \text{ for } i=1,\dots,k_P\} ,
\eeq

We propose two locally optimal strategies for the pursuer.


\subsection{Distance strategy}
The trajectories from the section~\ref{sec:hji} suggest that the pursuer must 
generally remain close to the evader. Otherwise, the evader can quickly hide behind obstacles.
A simple strategy for the pursuer is to move towards the evader:
\beq
\xp(t+\Delta t) &= \argmin_{x\in\pvalid(t)} \parrival\Big(x,\xe(t) \Big).
\eeq
That is, in the time increment $\Delta t$, the pursuer should pick the action that minimizes
its travel time to the evader's current position at time $t$. 

%In the next section, where we use search algorithms to refine policies,
%it is useful to quantify the utility of each action.
%To do so, define $p_\text{distance}:\Omega \times \free \times \free \to \mathbb{R}$ as the policy,
%which outputs a probability the agent should take an action, conditioned on the current player positions.
%We normalize using the \emph{softmax} function to generate the policy:
%\beq
%\norm &= \Big[\displaystyle{\sum_{x\in\pvalid(t)}} e^{ -\parrival(x,\xe(t))} \Big]^{-1}\\
%p_\text{distance}\big(x| (\xp(t),\xe(t))\big) &=  
%\begin{dcases}
%\norm e^{ -\parrival(x,\xe(t))}   & x \in \pvalid(t)\\
%0 & \text{otherwise}
%\end{dcases}
%\eeq

For the multiplayer game,  we propose a variant of the
Hausdorff distance, where max is replaced by a sum:
\begin{align*}
%\min_\pcontrol \sum_{i=1}^{k_P} \min_j \parrival[i]\Big( \xp_i(t+\Delta t),\xe_j(t) \Big)^2  +    \sum_{j=1}^{k_E} \min_i \parrival[i]\Big( \xp_i(t+\Delta t),\xe_j(t)\Big)^2 
%\argmin_{\substack{x_i\in\pvalid[i](t)\\i=1,\dots,k_P}} \   \sum_{i=1}^{k_P} \min_j \parrival[i]\Big( x_i,\xe_j(t) \Big)^2  +    \sum_{j=1}^{k_E} \min_i \parrival[i]\Big( x_i,\xe_j(t)\Big)^2 .
{\bf \parrival}({\bf x, \xe}(t)) := 
\frac{1}{2}\Big[ \sum_{i=1}^{k_P} \min_j \parrival[i]\Big( x_i,\xe_j(t) \Big)^2 \ \Big]^{1/2}  +  \frac{1}{2}\Big[  \sum_{j=1}^{k_E} \min_i \parrival[i]\Big( x_i,\xe_j(t)\Big)^2 \ \Big]^{1/2} .
\end{align*}
Informally, the first term encourages each pursuer to be close to an evader,
while the second term encourages a pursuer to be close to each evader.  The sum helps
to prevent ties. 
The optimal action according to the distance strategy is
\beq
%%%{\bf x^\ast} := (x_1^\ast,\dots,x_{k_P}^\ast)= \argmin_{\substack{x_i\in\pvalid[i](t)\\i=1,\dots,k_P}}{\bf \parrival}({\bf x, \xe}(t))  
%%%{\bf x^\ast} := (x_1^\ast,\dots,x_{k_P}^\ast)= \argmin_{{\bf x} \in \bfpvalid(t)}{\bf \parrival}({\bf x, \xe}(t))  
{\bfxp(t+\Delta t)} = \argmin_{{\bf x} \in \bfpvalid(t)}{\bf \parrival}({\bf x, \xe}(t))  
\eeq


In the next section, we will use search algorithms to refine policies.  Rather
than determining the \emph{best} action, it is useful to quantify the utility
of each action. To do so, define 
$p_\text{distance}:\Omega \times \free \times \dots \times \free \to \mathbb{R}$ as the policy,
which outputs a probability the agent should take an action, conditioned on the current player positions.
We normalize using the \emph{softmax} function to generate the policy:
%The corresponding policy for each pursuer is the marginal distribution corresponding to ${\bf x^\ast}$, in following sense.
%Define ${\bf x}^\ast_{-i} = (x_1^\ast,\dots,x_{i-1}^\ast,x_i,x_{i+1}^\ast,\dots,x_{k_P}^\ast)$. That is, replace the $i^{th}$ element in ${\bf x}^\ast$ with $x_i$.
%Then the distance policy for the $i^{th}$ pursuer is
\beq
\norm &= \Big[\displaystyle{\sum_{{\bf x}\in\bfpvalid(t)}} e^{ -{\bf \parrival}({\bf x},{\bf \xe}(t))}\Big]^{-1}\\
p_\text{distance}\big({\bf x}| ({\bf \xp}(t),{\bf \xe}(t))\big) &= 
\begin{dcases}
 \norm e^{ -{\bf \parrival}({\bf x},{\bf \xe}(t))}   & {\bf x} \in \bfpvalid(t)\\
0 & \text{otherwise}
\end{dcases}
\eeq


%In the case where there are more evaders than pursuers, the square term encourages a pursuer to stand in between evaders, rather than choosing to be close to an one.

For the discrete game with $\Delta t$ time increments,
one can enumerate the possible positions for each $\xp_i$ 
and evaluate the travel time to find the optimal control.
The arrival time function $\parrival[i](\cdot,\xe_j(t))$ to each $\xe_j$ at the current
time $t$ can be precomputed in $\bigo(m^d)$ time.  
In the general case, where each pursuer may have a different velocity field $\pspeed_i$, one
would need to compute $k_P$ arrival time functions.
If $a_{\Delta t}(P_i)$ is the
max number of possible actions each pursuer can make in $\Delta t$ increment, then the total
computational complexity for one move is 
$$ O\Big(k_P k_E m^d + \prod_{i=1}^{k_P} a_{\Delta_t}(P_i)\Big). $$

For the special case when the pursuers have the same $\pspeed$, the complexity reduces to
$$ O\Big(k_E m^d + \prod_{i=1}^{k_P} a_{\Delta_t}(P_i)\Big). $$



\subsection{Shadow strategy}

Recall that, for a stationary pursuer, the value function for the evader becomes
the Eikonal equation:
\beq
\espeed |\nabla_\xe \val|  &= 1 \qquad &\text{ on } \free\setminus\failset \\
\val(\xp,\xe) &= 0 &\qquad (\xp,\xe )\in \failset,
\eeq
whose solution is the travel time to the shadow set.
Define the time-to-occlusion as
\beq
\tstar(\xp,\xe^0) :=  \min_{\econtrol\in\admiss}  \min \{ t\ge 0 \ | \ \xe(0)=\xe^0 \ , \ (\xp,\xe(t)) \in \failset \ \} .
\eeq
It is the shortest time in which an evader at $\xe^0$ can be occluded from a stationary pursuer at $\xp$.
Thus, a reasonable strategy for the evader is to pick the action which brings it
closest to the shadow formed by the pursuer's position:
\beq
\xe(t+\Delta t) = \argmin_{y \in\evalid(t)} \tstar(\xp(t),y) .
\label{eq:evader-action}
\eeq
A conservative strategy for the pursuer, then, is to maximize time-to-occlusion, assuming that the evader can anticipate its actions:
\begin{align}
\tstar^\ast(x,\xe(t))  &= \min_{y \in\evalid(t)} \tstar(x,y)\\
\xp(t+\Delta t) &= \argmax_{x\in\pvalid(t)} \tstar^\ast(x) \label{eq:local-takei}.
\end{align}

%Define $p_\text{shadow}:\Omega \times \free \times \free \to \mathbb{R}$ as the 
%corresponding policy:
%\beq
%\norm &= \Big[\displaystyle{\sum_{x\in\pvalid(t)}} e^{ \tstar^\ast(x,\xe(t))} \Big]^{-1}\\
%p_\text{shadow}\big(x| (\xp(t),\xe(t))\big) &=  
%\begin{dcases}
%\norm e^{ \tstar^\ast(x,\xe(t))}   & x \in \pvalid(t)\\
%0 & \text{otherwise}
%\end{dcases}
%\eeq



\emph{Remark:} The strategy (\ref{eq:local-takei}) is a local variant of the static value
function proposed in \cite{takei2014efficient}.  In that paper, they suggest
using the static value function for feedback controls by moving towards the
globally optimal destination, and then recomputing at $\Delta t$ time
intervals. Here, we use the locally optimal action.

For multiple players, the game ends as soon as any evader is hidden from all pursuers. Define the time-to-occlusion for multiple players:
\beq
\bftstar({\bfxp},\bfxe^0):= \min_{\econtrol_i\in\admiss}  \min \{ t\ge 0 \ | \ \bfxe(0)=\bfxe^0 \ , \ (\bfxp,\bfxe(t)) \in \failset \ \} .
\eeq
Then, the strategy should consider the shortest time-to-occlusion among all possible evaders' actions in the $\Delta t$ time increment:
\beq
\bftstar^\ast({\bf x},{\bf \xe}(t))  &:= \min_{{\bf y} \in\bfevalid(t)} \bftstar({\bf x},{\bf y}) \\
\bfxp(t+\Delta t)  &= \argmax_{{\bf x}\in\bfpvalid(t)} \bftstar^\ast({\bf x},{\bf \xe}(t)).
 %%{\bf x}^\ast &= \argmax_{\substack{x_i\in\pvalid[i](t)\\i=1,\dots,k_P}} \bftstar^\ast({\bf x},{\bf \xe}(t)).
%\sup_{\pcontrol_i} \inf_{\econtrol_j}  \Big[ \inf_{j} \{ t | (\xp_i(t+\Delta t),\xe_j(T)) \in \failset \text{ for } i=1,\dots,k_P \Big]
\eeq
The corresponding shadow policy is:
\beq
\norm &= \Big[\displaystyle{\sum_{x\in\bfpvalid(t)}} e^{ \bftstar^\ast({\bf x},{\bf \xe}(t))}\Big]^{-1}\\
p_\text{shadow}\big({\bf x}| ({\bf \xp}(t),{\bf \xe}(t))\big) &= 
\begin{dcases}
 \norm e^{ \bftstar^\ast({\bf x},{\bf \xe}(t))}   & {\bf x} \in \bfpvalid(t)\\
0 & \text{otherwise}
\end{dcases}
\eeq


This strategy is computationally expensive. 
One can precompute the arrival time to each evader by solving an
Eikonal equation $\bigo(m^d)$.
For each combination of pursuer
positions, one must compute the joint visibility function  and corresponding
shadow function $\bigo(m^d)$.
Then the time-to-occlusion can be found by evaluating the precomputed
arrival times to find the minimum within the shadow set $\bigo(m^d)$.
The computational complexity for one move is
\beq O \Big( k_E m^d + m^d \cdot  \prod_{i=1}^{k_P} a_{\Delta t}(P_i) \Big). \eeq

%This strategy becomes very expensive as one increases the number of pursuers, or the velocity of each pursuer.
%With sufficient memory, one can precompute the visibilities for each pursuer's possible action,
%in which case, the complexity is

One may also consider alternating minimization strategies to achieve
\beq O \Big(k_E m^d + m^d \cdot  \sum_{i=1}^{k_P} a_{\Delta t}(P_i) \Big), \eeq
though we leave that for future work.

\subsection*{Blend strategy}



We have seen from $\ref{sec:hji}$ that optimal controls for the pursuer balance the
distance to, and visibility of, the evader. Thus a reasonable approach would be
to combine the distance and shadow strategies. However, it is not clear how
they should be integrated.  One may consider a linear combination, but 
the appropriate weighting depends on the game settings and environment.
Empirically, we observe that the product
of the policies provides promising results across a range of scenarios. Specifically, 
\beq
p_\text{blend} \propto p_\text{shadow} \cdot p_\text{distance}
\eeq


\subsection{Numerical results}

We present some representative examples of the local policies.
First, we consider the game with a circular obstacle, a single purser and single evader
whose speeds are $\pspeed=3$ and $\espeed=2$, respectively.
Figure~\ref{fig:traj-local-circle} illustrates the typical trajectories for each policy.
In general, the distance strategy leads the pursuer into a cat-and-mouse game
the with evader; the pursuer, when close enough, will jump to the evader's
position at the previous time step. The shadow strategy keeps the pursuer far
away from obstacles, since this allows it to \emph{steer the shadows} in the
fastest way.  The blend strategy balances the two approaches and resembles the
optimal trajectories based on the HJI equation in section~\ref{sec:hji}.


\begin{figure}[hptb]
\centering
\includegraphics[width=.42\textwidth,trim={0 0 0.1in 0},clip]{figures/traj/traj_seed_808_m_64_vP_3_vE_2_mcts_0_distance_vs_shadow_000.pdf}
\includegraphics[width=.42\textwidth,trim={0.1in 0 0 0},clip]{figures/traj/traj_seed_808_m_64_vP_3_vE_2_mcts_0_distance_vs_shadow_001.pdf}
\includegraphics[width=.42\textwidth,trim={0 0 0.1in 0},clip]{figures/traj/traj_seed_808_m_64_vP_3_vE_2_mcts_0_tstar_vs_shadow_000.pdf}
\includegraphics[width=.42\textwidth,trim={0.1in 0 0 0},clip]{figures/traj/traj_seed_808_m_64_vP_3_vE_2_mcts_0_tstar_vs_shadow_001.pdf}
\includegraphics[width=.42\textwidth,trim={0 0 0.1in 0},clip]{figures/traj/traj_seed_808_m_64_vP_3_vE_2_mcts_0_tstardist_vs_shadow_000.pdf}
\includegraphics[width=.42\textwidth,trim={0.1in 0 0 0},clip]{figures/traj/traj_seed_808_m_64_vP_3_vE_2_mcts_0_tstardist_vs_shadow_001.pdf}
\caption{Distance strategy (top) follows the evader closely, shadow strategy
(middle) stays far to gain better perspective, while the blend strategy
(bottom) strikes a balance.}


\label{fig:traj-local-circle}

\end{figure}

Next, we highlight the advantages of the shadow strategy with a
2 pursuer, 2 evader game on a map with two crescent-shaped obstacles.
The pursuer and evader speeds are $\pspeed=4$ and $\espeed=2$, respectively.
The openness of the environment creates large occlusions. The pursuers use the
shadow strategy to cooperate and essentially corner the evaders.
Figure~\ref{fig:traj-shadow-eyes} shows snapshots of the game. 
The distance strategy loses immediately since the green purser does not 
properly track the orange evader.





\begin{figure}[hptb]
\centering
\includegraphics[width=.42\textwidth,trim={0 .1in .1in 0},clip]{figures/traj/traj_eyes_seed_01_m_128_vP_4_vE_2_mcts_0_tstar_vs_shadow_000.pdf}
\includegraphics[width=.42\textwidth,trim={.1in .1in 0 0},clip]{figures/traj/traj_eyes_seed_01_m_128_vP_4_vE_2_mcts_0_tstar_vs_shadow_001.pdf}
\includegraphics[width=.42\textwidth,trim={0 .0 .1in .1in},clip]{figures/traj/traj_eyes_seed_01_m_128_vP_4_vE_2_mcts_0_tstar_vs_shadow_002.pdf}
\includegraphics[width=.42\textwidth,trim={.1in .0 0 .1in},clip]{figures/traj/traj_eyes_seed_01_m_128_vP_4_vE_2_mcts_0_tstar_vs_shadow_003.pdf}
\includegraphics[width=.42\textwidth]{figures/traj/traj_eyes_seed_01_m_128_vP_4_vE_2_mcts_0_distance_vs_shadow_000.pdf}
\caption{(Top 2 rows) The blue and green pursuers cooperate by using the shadow strategy. Green initially has responsibility of the orange
evader, but blue is able to take over. 
(Bottom) The distance strategy loses immediately.
}
\label{fig:traj-shadow-eyes}
\end{figure}


We present cases where the distance and shadow strategy fail in
Figure~\ref{fig:traj-failure}.  The evader tends to stay close to the obstacle,
since that enables the shortest path around the obstacle. Using the distance
strategy, the pursuer agressively follows the evader. The evader is able to
counter by quickly jumping behind sharp corners.  On the other hand, the shadow
strategy moves the pursuer away from obstacles to reduce the size of shadows.
As a consequence, the pursuer will generally be too far away from the evader
and eventually lose. In environments with many nonconvex obstacles, both
strategies will fail. 




\begin{figure}[hptb]
\centering
%\includegraphics[width=.45\textwidth]{figures/traj/traj_dice_seed_04_m_32_vP_3_vE_2_mcts_0_tstar_vs_shadow_001.pdf}
%\includegraphics[width=.45\textwidth]{figures/traj/traj_dice_seed_04_m_32_vP_3_vE_2_mcts_0_distance_vs_shadow_001.pdf}
%\includegraphics[width=.45\textwidth]{figures/traj/traj_eyes_seed_01_m_128_vP_4_vE_2_mcts_0_distance_vs_shadow_000.pdf}
\includegraphics[width=.45\textwidth]{figures/traj/traj_cross_seed_823_m_32_vP_4_vE_3_mcts_0_distance_vs_shadow_000.pdf}
\includegraphics[width=.45\textwidth]{figures/traj/traj_dice_seed_05_m_32_vP_3_vE_2_mcts_0_tstar_vs_shadow_000.pdf}
\caption{Failure modes for the local strategies. Blindly using the distance
strategy (left) allows the evader to exploit the sharp concavities. The
shadow strategy (right) keeps the pursuer far away to reduce the size of shadows, but often,
the pursuer is too far away to catch the evader.}
\label{fig:traj-failure} \end{figure}



Finally, we show that blending the shadow and distance strategies is very
effective in compensating for the shortcomings of each individual policy. 
The pursuers are able to efficiently track the evaders while maintain a safe distance.
Figure~\ref{fig:traj-blend-dice} shows an example with 2 pursuers and 2 evaders on
a map with multiple obstacles, where $\pspeed=3$ and $\espeed=2$.



\begin{figure}[hptb]
\centering
\includegraphics[width=.45\textwidth]{figures/traj/traj_dice_seed_04_m_32_vP_3_vE_2_mcts_0_tstardist_vs_shadow_000.pdf}
\includegraphics[width=.45\textwidth]{figures/traj/traj_dice_seed_04_m_32_vP_3_vE_2_mcts_0_tstardist_vs_shadow_001.pdf}
\includegraphics[width=.45\textwidth]{figures/traj/traj_dice_seed_04_m_32_vP_3_vE_2_mcts_0_tstardist_vs_shadow_002.pdf}
\includegraphics[width=.45\textwidth]{figures/traj/traj_dice_seed_04_m_32_vP_3_vE_2_mcts_0_tstardist_vs_shadow_003.pdf}
\caption{The pursuers (blue and green) 
are able to win by combining the distance and shadow strategy. The pursuers stay close, while maintaining
enough distance to avoid creating large shadow regions. The pursuers are slightly faster than the evaders.
}
\label{fig:traj-blend-dice}
\end{figure}




% show how distance can fail around crescent,
% show how tstar fails many obstacles
% show how blend is good at both

\section{Learning the pursuer policy}
\label{sec:learning-policy}

We propose a method for learning optimal controls for the pursuer, though our
methods can be applied to find controls for the evader as well.  Again, we
consider a discrete game, where each player's position is restricted on a grid,
and at each turn, the player can move to a new position within a neighborhood
determined by their velocity. All players move simultaneously. The game
termination conditions are checked at the end of each turn.  

We initialize a neural network which takes as input any game state,
and produces a policy and value pair. The policy is probability distribution
over actions. Unlike in section~\ref{sec:hji}, the value, in this context, is
an estimate of the likely winner given the input state. 


Initially the policy and value estimates are random.  We use Monte
Carlo tree search to compute refined policies.  We play the game using the
refined policies, and train the neural network to learn the refined policies.
By iterating in this feedback loop, the neural network continually learns to
improve its policy and value estimates. We train on games in various
environments and play games on-line on maps that were were not seen during the
training phase.


\subsection{Monte Carlo tree search}

In this section, we review the Monte Carlo tree search algorithm,
which allows the agent to plan ahead and refine policies. For clarity of notation,
we describe the single pursuer, single evader scenario, but the method applies to arbitrary
number of players.

Define the set of game states $\mathcal{S}:=\{(\xp,\xe)\in\free\times\free\}$ so that
each state $s\in\mathcal{S}$ characterizes the position of the players.
Let $\mathcal{A}\subseteq \free$ be the set of actions.
Let $\trans(s,a) : \mathcal{S}\times \mathcal{A} \to \mathcal{S}$ be the transition function
which outputs the state resulting from taking action $a$ at state $s$.
Let $\prior:\mathcal{S} \to \mathbb{R}^{m^d}\times[-1,1]$ be an evaluator function
which takes the current state as input and provides a policy and value estimate: $\prior(s)=(\vec{p},v)$.
Formally, Monte Carlo tree search is mapping takes as input the current state $s_0$, the evaluator function $\prior$, and a parameter $M$
indicating the number of search iterations: $\mcts(s_0,\prior;M)$.
It outputs a refined policy $\vec{\pi}^\ast$.

Algorithm \ref{alg:mcts} summarizes the MCTS algorithm.
At a high level, MCTS simulates game play starting from the current state,
keeping track of nodes it has visited during the search.
Each action is chosen according to a formula $U(s,a)$ which balances exploration and exploitation.
Simulation continues until the algorithm reaches a \emph{leaf node} $s_n$, a state which has not previously
been visited. At this point, we use the evaluator function $\prior(s_n)=(\vec{p},v)$ to estimate a policy
and value for that leaf node. The value $v$ is propagated to all parent nodes.
One iteration of MCTS ends when it reaches a leaf node.
MCTS keeps track of statistics that help guide the search. In particular
\begin{itemize}
\item $N(s,a)$: the number of times the action $a$ has been selected from state $s$
\item $W(s,a)$: the cumulative value estimate for each state-action pair
\item $Q(s,a)$: the mean value estimate for each state-action pair
\item $P(s,a)=(1-\varepsilon)p(a|s) + \varepsilon\eta$: the prior policy, computed by evaluating $\prior$. 
Dirichlet noise $\eta$ is added to allow a chance for each move to be chosen.
\item $U(s,a)=Q(s,a) + P(s,a) \frac{\sqrt{\sum_b N(s,b) }} {1+N(s,a)}$ is the \emph{upper confidence bound} \cite{rosin2011multi}. 
The first term exploits moves with high value, while the second term encourages moves that have not selected.
\end{itemize}

When all $M$ iterations are completed, the desired refined policy is proportional to $N(s_0,a)^{1/\tau}$,
where $\tau$ is a smoothing term.


\begin{algorithm}
\caption{Monte Carlo tree search: $\mcts(s_0,\prior,M)$} \label{alg:mcts}
\begin{algorithmic}
\State $N(s,a) \gets 0$ 
\State $Q(s,a) \gets 0$ 
\State $W(s,a) \gets 0$ 
\State visited = $\{ \emptyset \}$
\For{$i = 1,\dots,M $} 
  \State $n\gets0$
  \While{$s_n \notin$ visited}
	\State
	\If{ $\sum_b N(s_n,b)  > 0$}
    \State $a_n^\ast = \arg\max_a Q(s_n,a) + P(s_n,a) \frac{\sqrt{\sum_b N(s_n,b) }} {1+N(s_n,a)}$
	\Else
	\State  $a_n^\ast = \arg\max_a P(s_n,a)$
	\EndIf
    \State $s_{n+1} = \trans(s_n,a_n^\ast)$
    \State $n \gets n+1$
  \EndWhile

  \State $(p,v) = \prior(s_n)$
  \State $P(s_n,a) = (1-\varepsilon)p(a|s_n) + \varepsilon\eta$
  \State visited.append($s_n$)
  \For{$j = 0, \dots, n-1$}
    \State $N(s_j,a) \gets N(s_j,a_j^\ast) + 1$
    \State $W(s_j,a) \gets W(s_j,a_j^\ast) + v$
    \State $Q(s_j,a) \gets Q(s_j,a_j^\ast) / N(s_j,a_j^\ast)$
  \EndFor
\EndFor
\State $\pi^\ast(a|s_0) = N(s_0,a)^{1/\tau} / \sum_b N(s_0,b)^{1/\tau}$
\State \Return $\pi^\ast$
\end{algorithmic}
\end{algorithm}



\subsection{Policy and value network}

We use a convolutional neural network which takes in the game state
and produces a policy and value estimate.
Although the state can be completely characterized by the positions
of the players and the obstacles, the neural network requires more context in order to be
able to generalize to new environments.
We provide the following features as input to the neural network, each of which
is an $m\times m$ image:

\begin{itemize}
\item Obstacles as binary image
\item Player positions, a separate binary image for each player
\item Joint visibility of all pursuers, as a binary image
\item Joint shadow boundaries of all pursuers
\item Visibility from each pursuer's perspective, as a binary image
\item Shadow boundary from each pursuer's perspective
\item Valid actions for each player, as a binary image
\item Each evader's policy according to (\ref{eq:evader-action})
\end{itemize}

AlphaZero \cite{silver2017mastering2} suggests that training the policy and
value networks jointly improves performance.  We use a single network based on U-Net
\cite{ronneberger2015u}, which splits off to give output policy and value.

The input is $m\times m \times C_{\text{in}}$, where $C_{\text{in}}=2+4k_P+2k_E$ and $k_P,k_E$ are the number of
pursuers and evaders, respectively.
The U-Net consists of $\log_2(m)+1$ \emph{down-blocks}, followed by the same
number of \emph{up-blocks}.  
All convolution layers in the down-blocks and up-blocks use size 3 kernels.
Each down-block consists of input, conv, batch
norm, relu, conv, batch norm, residual connection from input, relu, followed by
downsampling with stride 2 conv, batch norm, and relu. A residual connection links
the beginning and end of each block, before downsampling.  The width
of each conv layer in the $l^{th}$ down-block is $l\cdot C_\text{in}$. Each
up-block is the same as the down-block, except instead of downsampling, we use
bilinear interpolation to upsample the image by a factor of 2. The upsampled
result is concatenated with the predownsampled output from the corresponding (same size)
down-block, followed by conv, batch norm, relu. The width of each conv layer in
the up-block is same as those in the down-block of corresponding size.

Then, the network splits into a policy and value head.
The policy head consists of $1\times 1$ conv with width 8, batch norm, relu, and
$1\times 1$ conv with width $k_P$. The final activation layer is a softmax to output $p\in \mathbb{R}^{m\times m \times k_P}$, a policy for each pursuer.
The value head is similar, with $1\times 1$ conv with width 8, batch norm, relu, and
$1\times 1$ conv with width 1. The result passes through a tanh activation and
average pooling to output a scalar $v\in[-1,1]$.


\subsection{Training procedure}
Since we do not have the true value and policy, we cannot train the networks
in the usual supervised fashion. Instead, we use MCTS to generate refined policies,
which serve as the training label for the policy network. 
Multiple games are played with actions selected according to MCTS refined policies.
The game outcomes act as the label for the value for each state in the game.
We train over various maps consisting of 2-7 obstacles, including circles, ellipses, squares,
and tetrahedrons.

More specifically,
let $\prior_\theta(s) $ be the neural network parameterized by $\theta$, which takes a state $s$ as input, and outputs a policy $\vec{\pi}_\theta(s)$ and value $v_\theta(s)$.
Let $s_j(0)$ be the initial positions.
For $j=1,\dots,J$, play the game using MCTS:
\begin{align}
\vec{\pi}_j(a|s_j(k)) &= \text{MCTS}(s_j(k), f_\theta; M)   \\
s_j(k+1) &= \arg\max_a \vec{\pi}_j^\ast(a|s_j(k))
\end{align}

for $k=0,\dots,K_j$. The game ends at 
\beq
K_j = \inf\{k | s_j(k) \in \mathcal{T}_\text{end}\}
\eeq

Then the "true" policy and value are
\begin{align}
\vec{\pi}_j^\ast(k) &= \vec{\pi}_j(\cdot|s_j(k))\\
v^\ast_j(k)&= 
\begin{cases} 
1  & K_j > K_\text{max}  \\
-1  & \text{otherwise}
\end{cases}
\end{align}


The parameters $\theta$ of the neural network
are updated by stochastic gradient descent (SGD) on the loss function:
\beq 
\min_\theta \sum_{j=1}^J \sum_{k=0}^{K_j}  L_{\text{policy}} & \Big(\vec{\pi}_\theta(s_j(k)) , \vec{\pi}_j^\ast(k) \Big) + L_\text{value} \Big(v_\theta(s_j(k)),v_j^\ast(k)\Big)\\
L_\text{policy}(\vec{p},\vec{q}) &= -\vec{p} \cdot \log \vec{q} \\
L_\text{value}(p,q) &= (p-q)^2 \\
\eeq

We use a learning rate of $0.001$ and the Adam optimizer \cite{kingma2014adam}.

\subsection{Numerical results}

A key difficulty in learning a good policy for the pursuer
is that it requires a good evader. If the evader is static,
then the pursuer can win with any random policy.

During training and evaluation, the game is played with the evader moving
according to (\ref{eq:evader-action}).  Although all players move
simultaneously, our MCTS models each team's actions sequentially, with the
pursuers moving first. This is conservative towards the pursuers, since the
evaders can counter.

We train using a single workstation with 2 Intel Xeon CPU E5-2620 v4 2.10GHz
processors and a single NVidia 1080-TI GPU.  For simplicity, $\pspeed$ and $\espeed$ are
constant, though it is straightforward to have spatially varying
velocity fields.  We use a gridsize of $m=16$. We set $K_{\text{max}}=100$ and
$M=1000$ MCTS iterations per move.  One step of training consists of playing
$J=64$ games and then training the neural network for 1 epoch based on training
data for the last 10 steps of training.  Self-play game data is generated in
parallel, while network training is done using the GPU with batch size 128. The total
training time is 1 day.

The training environments consist of between 2 to 6 randomly oriented obstacles,
each uniformly chosen from the set of ellipses, diamonds, and rectangles. We emphasize
that the environments shown in the experiments are not in the training set.

We compare our trained neural network against uniform random and dirichlet
noise-based policies, as well as the local policies from
section~\ref{sec:locally}.  In order to draw a fair comparison, we make sure
each action requires the same amount of compute time.  Each MCTS-based move in
the 2 player game takes 4 secs while the multiplayer game takes about 10 secs
per move, on average.  Since the noise-based policies require less overhead,
they are able to use more MCTS iterations.  The shadow strategies become very
expensive as more players are added. For the 1v1 game, we use $\hat{M}=1000$,
while the 2v2 game can only run for $\hat{M}=250$ in the same amount of time as
the Neural Net. 
Specifically,
\begin{itemize}
\item Distance strategy
\item Shadow strategy
\item Blend strategy
\item $\mcts(\cdot,\prior_\text{distance},1000)$ where $\prior_\text{distance}(s) = (p_\text{distance},0)$.
\item $\mcts(\cdot,\prior_\text{shadow},\hat{M})$ where $\prior_\text{shadow}(s) = (p_\text{shadow},0)$.
\item $\mcts(\cdot,\prior_\text{blend},\hat{M})$ where $\prior_\text{blend}(s) = (p_\text{blend},0)$.
\item $\mcts(\cdot,\prior_\mu,2000)$ where $\prior_\nu(s) = (\text{Uniform},0)$.
\item $\mcts(\cdot,\prior_\eta,2000)$ where $\prior_\eta(s) = (\text{Dir}(0.3),0)$.
\item $\mcts(\cdot,\prior_\theta,1000)$ where $\prior_\theta$ is the trained Neural Network
\end{itemize}



\subsection*{Two players}
As a sanity check, we show an example on a single circular obstacle with a
single pursuer and single evader.  As we saw from the previous section, the
pursuer needs to be faster in order to have a chance at winning. We let
$\pspeed=2$ and $\espeed=1$.
Figure~\ref{fig:nnet-traj-circle} shows an example trajectory using Neural Net.
The neural network model gives reasonable policies. 
Figure~\ref{fig:nnet-traj-v} shows an adversarial human evader playing against the Neural Net pursuer,
on a map with two obstacles. The pursuer changes strategies depending on the shape of the obstacle.
In particular, near the corners of the "V" shape, it maintains a safe distance rather than blindly following
the evader.

\begin{figure}[hptb]
\centering
\includegraphics[width=.45\textwidth]{figures/traj/traj_seed_01_m_16_vP_2_vE_1_mcts_1000_nnet_vs_shadow_000.pdf}
\includegraphics[width=.45\textwidth]{figures/traj/traj_seed_01_m_16_vP_2_vE_1_mcts_1000_nnet_vs_shadow_001.pdf}
\includegraphics[width=.45\textwidth]{figures/traj/traj_seed_01_m_16_vP_2_vE_1_mcts_1000_nnet_vs_shadow_002.pdf}
\includegraphics[width=.45\textwidth]{figures/traj/traj_seed_01_m_16_vP_2_vE_1_mcts_1000_nnet_vs_shadow_003.pdf}
\caption{Snapshots of the trajectory for the Neural Net pursuer around a circular obstacle. 
The pursuer (blue) tracks the evader (red) while maintaining a safe distance.
View from left to right, top to bottom.
Stars indicate the initial positions, and the black line (of sight) connects the players at the end of each time interval.} 
\label{fig:nnet-traj-circle}

\end{figure}


\begin{figure}[hptb]
\centering
\includegraphics[width=.45\textwidth]{figures/traj/traj_vshape_seed_82_m_16_vP_2_vE_1_mcts_0_nnet_vs_shadow_000.pdf}
\includegraphics[width=.45\textwidth]{figures/traj/traj_vshape_seed_82_m_16_vP_2_vE_1_mcts_0_nnet_vs_shadow_001.pdf}
\includegraphics[width=.45\textwidth]{figures/traj/traj_vshape_seed_82_m_16_vP_2_vE_1_mcts_0_nnet_vs_shadow_002.pdf}
\includegraphics[width=.45\textwidth]{figures/traj/traj_vshape_seed_82_m_16_vP_2_vE_1_mcts_0_nnet_vs_shadow_003.pdf}
\caption{Trajectory for the Neural Net pursuer against an adversarial human evader on a map with two obstacles. The pursuer
transitions between following closely, and leaving some space, depending on the shape of the obstacle.} 
\label{fig:nnet-traj-v}

\end{figure}



%\begin{figure}[hptb]
%\centering
%\includegraphics[width=.45\textwidth]{figures/traj/traj_dice_seed_05_m_16_vP_2_vE_1_mcts_1000_nnet_vs_shadow_000.pdf}
%\includegraphics[width=.45\textwidth]{figures/traj/traj_dice_seed_05_m_16_vP_2_vE_1_mcts_1000_nnet_vs_shadow_001.pdf}
%\includegraphics[width=.45\textwidth]{figures/traj/traj_dice_seed_05_m_16_vP_2_vE_1_mcts_1000_nnet_vs_shadow_002.pdf}
%\includegraphics[width=.45\textwidth]{figures/traj/traj_dice_seed_05_m_16_vP_2_vE_1_mcts_1000_nnet_vs_shadow_003.pdf}
%\caption{Snapshots of the trajectory for the NNet pursuer around a circular obstacle. View from left to right, top to bottom.
%Stars indicate the initial positions, and the black line connects the players at the end of each time interval.} 
%\label{fig:nnet-traj-dice}
%
%\end{figure}

In order to do a more systematic comparison, we run multiple games
over the same map and report the game time statistics for each method.
We fix the pursuer's position at $(1/2,1/4)$ and vary the evader's initial location within the free space.
Figure~\ref{fig:value-slice-setup} shows the setup for the two maps considered for the statistical studies in this section.
One contains a single circle in the center, as we have seen previously. The other one contain 5 circular obstacles,
though the one in the center has some extra protrusions.

Figure~\ref{fig:value-slice-1v1dice} shows an image corresponding the the length of the game
for each evader position; essentially, it is a single slice
of the value function for each method.
Table~\ref{tab:1v1dice} shows the number of games won. Shadow strategy particularly benefits
from using MCTS for policy improvements, going from 16\% to 67.15\% win rate. Our neural network
model outperforms the rest with a 70.8\% win rate.


\begin{figure}[hptb]
\centering
\includegraphics[width=.45\textwidth]{figures/value_slices/value_2v2circle_setup.png}
\includegraphics[width=.45\textwidth]{figures/value_slices/value_2v2dice_setup.png}
\caption{Setup for computing a slice of the value function for the circular obstacle (left) and 5 obstacle map (right). The pursuer's initial position is fixed (blue) while the
evader's changes within the free space.} 
\label{fig:value-slice-setup}
\end{figure}


\begin{figure}[hptb]
\centering
\includegraphics[width=.3\textwidth]{figures/value_slices/value_1v1dice_dist.png}
\includegraphics[width=.3\textwidth]{figures/value_slices/value_1v1dice_tstar.png}
\includegraphics[width=.3\textwidth]{figures/value_slices/value_1v1dice_tstardist.png}
\includegraphics[width=.3\textwidth]{figures/value_slices/value_1v1dice_dist1000.png}
\includegraphics[width=.3\textwidth]{figures/value_slices/value_1v1dice_tstar1000.png}
\includegraphics[width=.3\textwidth]{figures/value_slices/value_1v1dice_tstardist1000.png}
\includegraphics[width=.3\textwidth]{figures/value_slices/value_1v1dice_uniform2000.png}
\includegraphics[width=.3\textwidth]{figures/value_slices/value_1v1dice_dir2000.png}
\includegraphics[width=.3\textwidth]{figures/value_slices/value_1v1dice_nnet1000.png}
\caption{One slice of the "value" function for single pursuer, single evader game with 5 obstacles. Bright spots
indicate that the pursuer won the game if that pixel was the evader's initial position.}
\label{fig:value-slice-1v1dice}
\end{figure}




\begin{table}[]
\caption{Game statistics for the 1 pursuer vs 1 evader game with 5 circular obstacles, where $\pspeed=2$ and $\espeed=1$.\vspace{1em}}
\label{tab:1v1dice}
\begin{tabular}{l|ccc}
Method          & Win \% (137 games) & Average game time                 \\   % & Average loss time \\
\hline
Distance                         &52.55       & 53.56         \\   % & 4.7             \\
Shadow                           &16.06       & 22.36         \\   % & 7.2             \\
Blend                            &63.50       & 64.45         \\   % & 7.3             \\
MCTS($\cdot$, Distance; 1000)    &55.47       & 62.40         \\   % & 12.2            \\
MCTS($\cdot$, Shadow; 1000)      &67.15       & 69.45         \\   % & 6.3             \\
MCTS($\cdot$, Blend; 1000)       &58.39       & 63.27         \\   % & 4.4             \\
MCTS($\cdot$, Uniform; 2000)     &60.58       & 65.84         \\   % & 5.3             \\
MCTS($\cdot$, Dirichlet; 2000)   &65.69       & 69.02         \\   % & 7.0             \\
MCTS($\cdot$, Neural Net; 1000)  &70.80       & 71.61         \\   % & 4.7            
\end{tabular}                     
\end{table}
% OLD, somehow incorrect
%66.42                     & 67.30
%5.84                      & 20.50
%73.72                     & 74.45
%75.18                     & 78.69
%80.29                     & 82.02
%73.72                     & 77.18
%60.58                     & 65.83
%65.69                     & 69.02
%83.21                     & 83.65


\subsection*{Multiple players}
Next, we consider the multiplayer case with 2 pursuers and 2 evaders on a circular obstacle map
where $\pspeed=2$ and $\espeed=2$. 
Even on a $16\times16$ grid, the computation of the corresponding feedback value function 
would take several days.
Figure~\ref{fig:nnet-traj-circle-multi} shows a sample trajectory. Surprisingly, the neural network has learned
a smart strategy. Since there is only a single obstacle, it is sufficient for each
pursuer to guard one opposing corner of the map. Although all players have the same speed, it is possible
to win.

\begin{figure}[phtb]
\centering
\includegraphics[width=.45\textwidth]{figures/traj/traj_seed_06_m_16_vP_2_vE_2_mcts_1000_nnet_vs_shadow_000.pdf}
\includegraphics[width=.45\textwidth]{figures/traj/traj_seed_06_m_16_vP_2_vE_2_mcts_1000_nnet_vs_shadow_001.pdf}
\includegraphics[width=.45\textwidth]{figures/traj/traj_seed_06_m_16_vP_2_vE_2_mcts_1000_nnet_vs_shadow_002.pdf}
\includegraphics[width=.45\textwidth]{figures/traj/traj_seed_06_m_16_vP_2_vE_2_mcts_1000_nnet_vs_shadow_003.pdf}
%\includegraphics[width=.45\textwidth]{figures/traj/traj_seed_03_m_16_vP_2_vE_2_mcts_1000_nnet_vs_shadow_004.pdf}
\caption{Trajectories for the multiplayer game played using NNet around a circle. Pursuers are blue and green, while evaders are red and orange.
Blue has learned the tactic of remaining stationary in the corner, while green manages the opposite side.
The evaders movements are sporadic because there is no chance of winning; there are no shadows in which to hide.} 
\label{fig:nnet-traj-circle-multi}

\end{figure}



Figure~\ref{fig:value-slice-2v2circle} shows a slice of the value function, where 3 players' positions are fixed,
and one evader's position varies.
Table~\ref{tab:2v2circle} shows the game statistics.
Here, we see some deviation from the baseline. As the number of players increase,
the number of actions increases. It is no longer sufficient to use random sampling.
The neural network is learning useful strategies to help guide the
Monte Carlo tree search to more significant paths. The distance and blend strategies
are effective by themselves. MCTS helps improve performance for Distance. However, 250 iterations is
not enough to search the action space, and actually lead to poor performance for Blend and Shadow.
For this game setup, MCTS(Distance,1000) performs the best with a 73.5\% win rate, followed by 
Blend with 65.4\% and Neural Net with 59.9\%. Although the trained network is not the best
in this case, the results are very promising. We want to emphasize that the model was trained with no prior
knowledge. Given enough offline time and resources, we believe the proposed approach can scale to larger grids and
learn more optimal policies than the local heuristics.


\begin{figure}[phtb]
\centering
\includegraphics[width=.3\textwidth]{figures/value_slices/value_2v2circle_dist.png}
\includegraphics[width=.3\textwidth]{figures/value_slices/value_2v2circle_tstar.png}
\includegraphics[width=.3\textwidth]{figures/value_slices/value_2v2circle_tstardist.png}
\includegraphics[width=.3\textwidth]{figures/value_slices/value_2v2circle_dist1000.png}
\includegraphics[width=.3\textwidth]{figures/value_slices/value_2v2circle_tstar250.png}
\includegraphics[width=.3\textwidth]{figures/value_slices/value_2v2circle_tstardist250.png}
\includegraphics[width=.3\textwidth]{figures/value_slices/value_2v2circle_uniform2000.png}
\includegraphics[width=.3\textwidth]{figures/value_slices/value_2v2circle_dir2000.png}
\includegraphics[width=.3\textwidth]{figures/value_slices/value_2v2circle_nnet1000.png}
\caption{One slice of the value function for 2 pursuer, 2 evader game on the circular obstacle.}
\label{fig:value-slice-2v2circle}
\end{figure}


\begin{table}[]
\caption{Game statistics for the 2 pursuer vs 2 evader game with a circular obstacle.\vspace{1em}}
\label{tab:2v2circle}
\begin{tabular}{l|ccc}
Method          & Win \% (162 games) & Average game time                 \\   % & Average loss time \\
\hline
Distance                        & 56.8                     & 58.8        \\   % & 4.7             \\
Shadow                          & 46.3                     & 50.1        \\   % & 7.2             \\
Blend                           & 65.4                     & 67.9        \\   % & 7.3             \\
MCTS($\cdot$, Distance; 1000)    & 73.5                     & 76.6        \\   % & 12.2            \\
MCTS($\cdot$, Shadow; 250)       & 40.7                     & 44.5        \\   % & 6.3             \\
MCTS($\cdot$, Blend; 250)        & 00.0                     &  4.4        \\   % & 4.4             \\
MCTS($\cdot$, Uniform; 2000)     & 00.0                     &  5.3        \\   % & 5.3             \\
MCTS($\cdot$, Dirichlet; 2000)   & 27.8                     & 32.8        \\   % & 7.0             \\
MCTS($\cdot$, Neural Net; 1000)  & 59.9                     & 61.7        \\   % & 4.7            
\end{tabular}
\end{table}


% HERE WE HAVE 5 OBSTACLE RESULTS, BUT I NEED TO RETRAIN NNET SO WE CAN HAVE vP3, vE2.
% ACTUALLY THE MAP IS TOO SMALL TO BE INTEReSTING
\iffalse
We repeat the experiment for the more complicated map with 5 obstacles,
with $\pspeed=\espeed=2$, and show the results in
Figure~\ref{fig:value-slice-2v2dice} and Table~\ref{tab:2v2dice}. The map 
is much more difficult and the evader generally wins. For this particular map and game setting,
where all players
Distance has a slight edge over the other strategies, though



\begin{table}[]
\caption{Game statistics for the 2 pursuer vs 2 evader game with 5 obstacles.\vspace{1em}}
\label{tab:2v2dice}
\begin{tabular}{l|ccc}
Method          & Win \% (137 games) & Average game time                 \\ %  & Average loss time \\
\hline
Distance                        & 6.6                     & 8.89         \\ %  & 2.49             \\
Shadow                          & 0                       & 2.68         \\ %  & 2.68            \\
Blend                           & 0.7                     & 3.95         \\ %  & 3.25           \\
MCTS($\cdot$,Distance; 1000)    & 0.7                     & 3.77         \\ %  & 3.06           \\
MCTS($\cdot$,Shadow; 250)       & 0                       & 2.24         \\ %  & 2.24            \\
MCTS($\cdot$,Blend; 250)        & 0                       & 1.77         \\ %  & 1.77            \\
MCTS($\cdot$,Uniform; 2000)     & 0                       & 2.10         \\ %  & 2.10            \\
MCTS($\cdot$,Dirichlet; 2000)   & 0                       & 2.26         \\ %  & 2.26            \\
MCTS($\cdot$,Neural Net; 1000)  & 0                       & 3.0           %  & 3.0            
\end{tabular}
\end{table}




\begin{figure}[phtb]
\centering
\includegraphics[width=.3\textwidth]{figures/value_slices/value_2v2dice_dist.png}
\includegraphics[width=.3\textwidth]{figures/value_slices/value_2v2dice_tstar.png}
\includegraphics[width=.3\textwidth]{figures/value_slices/value_2v2dice_tstardist.png}
\includegraphics[width=.3\textwidth]{figures/value_slices/value_2v2dice_dist1000.png}
\includegraphics[width=.3\textwidth]{figures/value_slices/value_2v2dice_tstar250.png}
\includegraphics[width=.3\textwidth]{figures/value_slices/value_2v2dice_tstardist250.png}
\includegraphics[width=.3\textwidth]{figures/value_slices/value_2v2dice_uniform2000.png}
\includegraphics[width=.3\textwidth]{figures/value_slices/value_2v2dice_dir2000.png}
\includegraphics[width=.3\textwidth]{figures/value_slices/value_2v2dice_nnet1000.png}
\caption{One slice of the value function for the dice}
\label{fig:value-slice-2v2dice}
\end{figure}
\fi




Figure~\ref{fig:mcts-stats-multi} shows a comparison of the depth of search for
$M=1000$ MCTS iterations.  Specifically, we report depth of each leaf node, as
measured by game time. To be fair, we allow the uniform and dirichlet baselines 
to run for 2000 MCTS iterations to match the runtime needed for 1 move.  Also,
the shadow strategies are extremely costly, and can only run 250 MCTS
iterations in the same amount of time. However, we show the statistics for
$M=1000$ to gain better insights.  Ideally, a good search would balance breadth
and depth.  The neural network appears to search further than the baselines. Of
course, this alone is not sufficient to draw any conclusions. For example, a
naive approach could be a depth-first search. 

In Figure~\ref{fig:mcts-stats}, we show a similar chart for the single pursuer,
single evader game with a circular obstacle. In this case, the game is
relatively easy, and all evaluator functions are comparable.



   \begin{figure}[hptb]
      \centering
      \includegraphics[width=.45\textwidth,trim={0 0.15in 0 0},clip]{figures/mcts_stats/seed_02_m_16_vP_2_vE_2_mcts_2000_uniform_vs_shadow.pdf} \quad
      \includegraphics[width=.45\textwidth,trim={0 0.15in 0 0},clip]{figures/mcts_stats/seed_02_m_16_vP_2_vE_2_mcts_2000_dirichlet_vs_shadow.pdf}\\[.5em]
      \includegraphics[width=.45\textwidth,trim={0 0.15in 0 0},clip]{figures/mcts_stats/seed_02_m_16_vP_2_vE_2_mcts_1000_distance_vs_shadow.pdf} \quad
      \includegraphics[width=.45\textwidth,trim={0 0.15in 0 0},clip]{figures/mcts_stats/seed_02_m_16_vP_2_vE_2_mcts_1000_tstar_vs_shadow.pdf} \\[.5em]
      \includegraphics[width=.45\textwidth,trim={0 0in 0 0},clip]{figures/mcts_stats/seed_02_m_16_vP_2_vE_2_mcts_1000_tstardist_vs_shadow.pdf} \quad
      \includegraphics[width=.45\textwidth,trim={0 0in 0 0},clip]{figures/mcts_stats/seed_02_m_16_vP_2_vE_2_mcts_1000_nnet_vs_shadow.pdf} \quad

	  \caption{Histogram of leaf node depth for MCTS using various evaluator
functions for the multiplayer game around a circular obstacle.  The colors show
increments of 100 iterations. The multiplayer game has a much larger action
space, making tree search difficult. The neural network appears to search deeper
into the tree.} 

\label{fig:mcts-stats-multi}

\end{figure}


   \begin{figure}[hptb]
      \centering
      \includegraphics[width=.45\textwidth,trim={0 0.15in 0 0},clip]{figures/mcts_stats/seed_00_m_16_vP_2_vE_1_mcts_2000_uniform_vs_shadow.pdf} \quad
      \includegraphics[width=.45\textwidth,trim={0 0.15in 0 0},clip]{figures/mcts_stats/seed_00_m_16_vP_2_vE_1_mcts_2000_dirichlet_vs_shadow.pdf}\\[.5em]
      \includegraphics[width=.45\textwidth,trim={0 0.15in 0 0},clip]{figures/mcts_stats/seed_00_m_16_vP_2_vE_1_mcts_1000_distance_vs_shadow.pdf} \quad
      \includegraphics[width=.45\textwidth,trim={0 0.15in 0 0},clip]{figures/mcts_stats/seed_00_m_16_vP_2_vE_1_mcts_1000_tstar_vs_shadow.pdf} \\[.5em]
      \includegraphics[width=.45\textwidth,trim={0 0.00in 0 0},clip]{figures/mcts_stats/seed_00_m_16_vP_2_vE_1_mcts_1000_tstardist_vs_shadow.pdf} \quad
      \includegraphics[width=.45\textwidth,trim={0 0.00in 0 0},clip]{figures/mcts_stats/seed_00_m_16_vP_2_vE_1_mcts_1000_nnet_vs_shadow.pdf} \quad

	  \caption{Histogram of leaf node depth for MCTS using various evaluator
functions for the single pursuer vs single evader game around a circular
obstacle.  The colors show increments of 100 iterations. The game is relatively easy
and thus all algorithms appear comparable. Note that Uniform and Dirichlet are allowed 2000 MCTS iterations,
since they require less overhead to run.} 

\label{fig:mcts-stats}
\end{figure}








\section{Conclusion and future work}
We proposed three approaches for approximating optimal controls for the
surveillance-evasion game. When there are few players and the grid size is
small, one may compute the value function via the Hamilton-Jacobi-Isaacs
equations. The offline cost is immense, but on-line game play is very
efficient. The game can be played on the continuously in time and space, since
the controls can be interpolated from the value function. However, the value
function must be recomputed if the game settings, such as the obstacles or player
velocities, change.

When there are many players, we proposed locally optimal strategies for the
pursuer and evader. There is no offline preprocessing. All computation is done
on-line, though the computation does not scale well as the velocities or number
of pursuers increases. The game is discrete in time and space.

Lastly, we proposed a reinforcement learning approach for the 
multiplayer game. The offline training time can be enormous, but on-line game play
is very efficient and scales linearly with the number of players. The game is played
in discrete time and space, but the neural network model generalizes to
maps not seen during training. Given enough computational resources,
the neural network has the potential to approach the optimal controls
afforded by the HJI equations, while being more efficient than the local strategies.


There are many avenues to explore for future research.  
We are working on the extension of our reinforcement learning approach to 3D,
which is straight-forward, but requires more computational resources.
Figure~\ref{fig:3dseg} shows an example surveillance-evasion game in 3D. Along
those lines, a multi-resolution scheme is imperative for scaling to higher
dimensions and resolutions.  One may also consider different game objectives,
such as seeking out an intially hidden evader, or allowing brief moments of
occlusion.  


   \begin{figure}[hptb]
	\vspace{1em}
      \centering
      %\fbox{\includegraphics[width=.65\textwidth]{figures/3d_seg_crop.png}}
      \includegraphics[width=.65\textwidth]{figures/3d_seg_crop.png}
	  \caption{A snapshot of a 3D surveillance-evasion game around a sphere.} 
\label{fig:3dseg}
\end{figure}



% in thesis but removing for arxiv
\iffalse
\subsection{The surveillance-constrained patrol problem}

In \cite{bharadwaj2019strategy}, we considered a surveillance-constrained
patrol problem where a pursuer must optimize short-term visibility of the
environment, with the constraint that 
it must always keep the evader within its line-of-sight. In this section, we briefly
review the ideas in that paper, and mention a direction for future work which combines
the ideas presented in Chapters~\ref{chap:exploration} and \ref{chap:surveillance}.

The game is played in discrete space and time. We assume that
both players have a map of the environment; the pursuer must be faster than the
evader, otherwise it may not have any flexibility to do anything other than the
surveillance constraint.
Formally, let $K\in \mathbb{N}$. Short-term visibility means that the pursuer's
visibility of the environment at time $t$ is only valid for $K$ time steps, after which those
portions are assumed to be occluded again. Define the short-term visibility set
\beq
\Omega_{i-K}^i := \bigcup_{j=i-K}^i \visset(\xp_j)
\eeq
As in Chapter~\ref{chap:exploration}, one may define the gain function
\begin{equation}
g^K(x;\Omega_{i-K}^i) := |   \visset_x  \cup \Omega_{i-K}^i| - |\Omega_{i-K}^i|, \label{eq:short-gain-func} 
\end{equation}
Then the problem can be stated as a constrained optimization problem:
\beq
&\max_{\xp(i)} g^K({\xp(i)};\Omega_{i-K}^i) \\ &\text{ subj. to } \xe(t) \in \visset(\xp(t)) \text{ for } t\ge i
\eeq
The constraint is challenging since it needs to hold for all future time.
In \cite{bharadwaj2019strategy}, we satisfy the constraint by using reactive synthesis tools
to precompute the \emph{feasible set} 
$$\mathcal{F} :=\{ (\xp(0),\xe(0)) |\xe(t) \in \visset(\xp(t)) \text{ for } t\ge0\} ,$$
which is the set of positions from which it is possible to maintain the surveillance requirement for all time.
The problem can now be reformulated as
\beq
&\max_{\xp(i)} g^K({\xp(i)};\Omega_{i-K}^i) \\&\text{ subj. to } (\xp(i),\xe(i)) \in \mathcal{F},
\eeq
where the optimization of the objective function can be done greedily during game-play.
Figure~\ref{fig:patrol} shows snapshots from an example surveillance-constrained patrol game.

% The reactive synthesis tools are flexible in being able to handle a wide range of temporal surveillance objectives. However, the complexity is $\bigo(m^{2kd})$, where $k$ is the number of players, and $d$ is the number of dimensions.


For future work, we envision the use of the value function from section~\ref{sec:hji} to compute
the feasible set for the \emph{continuous} version of the game.
Optimization of $g^K$ can be done using a greedy approach powered by a convolutional neural network, as in
Chapter~\ref{chap:exploration}. Monte Carlo tree search may also help refine strategies and generate
causually relevant training data that surpasses the one-step lookahead policy afforded by the greedy algorithm.

\begin{figure}[ht!]

    %\begin{minipage}{5.0cm}
        \subfloat[$t=0$]{
            \includegraphics[width=0.3\textwidth]{figures/patrol/casestudyfigs_high_res/frame_green_0000.png}
        }
            \subfloat[$t=10$ \label{fig:case1t10}]{
            \includegraphics[width=0.3\textwidth]{figures/patrol/casestudyfigs_high_res/frame_green_0010.png}
        }
            \subfloat[$t=16$ \label{fig:case1t16}]{
            \includegraphics[width=0.3\textwidth]{figures/patrol/casestudyfigs_high_res/frame_green_0016.png}
        }\\
            \subfloat[$t=20$ \label{fig:case1t20}]{
            \includegraphics[width=0.3\textwidth]{figures/patrol/casestudyfigs_high_res/frame_green_0020.png}
        }
            \subfloat[$t=24$ \label{fig:case1t24}]{
            \includegraphics[width=0.3\textwidth]{figures/patrol/casestudyfigs_high_res/frame_green_0024.png}
        }
            \subfloat[$t=33$ \label{fig:case1t33}]{
            \includegraphics[width=0.3\textwidth]{figures/patrol/casestudyfigs_high_res/frame_green_0033.png}
        }

    %\end{minipage}



	\caption{Example of the surveillance-constrained patrol game with a single
pursuer (blue) and single evader (orange). The pursuer tries to optimize
short-term visibility of the environment when possible, but must always
maintain visibility of the evader.  The green cells correspond to the pursuer's
planned path to a vantage point.  Obstacles are shown in red, with occlusions
in black.}

    \label{fig:patrol}
\end{figure}

\fi



==> related_works.tex <==
    
Convolutional Neural Networks (CNNs) have become the undisputed
state-of-the-art for image classification tasks, where an input image has to be
binned into one of $n$ classes. The major advantage of CNNs is that it uses a
learned classifier over learned set of features. This has been empirically
shown to be better than the previous state-of-the-art, where learned
classifiers were trained on hand-tuned features.  CNNs are appealing due to
their efficiency, translational invariance, and representational capacity.  The
drawback is that training requires lots of data and computational time.

A neural network architecture consists of various layers, which map the input
to the desired output. There are many architectures; the most popular image
classification networks are Alex-Net \cite{krizhevsky2012imagenet} , VGG
\cite{simonyan2014very}, Inception \cite{szegedy2015going}, and ResNet
\cite{he2016deep}.  More recently, fully convolutional neural networks have
shown promise in dense inference tasks, which requires an output for each
input. We base our CNN on U-Net \cite{ronneberger2015u}, which has a simple
design and efficiently aggregates information across multiple scales.


\subsubsection*{Layers}

Given an input vector-valued image $I\in\mathbb{R}^{W_{in}\times H_{in}\times C_{in}}$,
a CNN defines a transformation $f:I\to P\in\mathbb{R}^{W_{out}\times H_{out}\times C_{out}}$.
Usually $P$ will be a probability map, i.e. each entry in $P$ contains
the probability that the corresponding pixel belongs to each of the
$C_{out}$ classes. This transformation is a composition of linear
and nonlinear functions. A CNN has multiple layers of each of these.
Some of the most common functions include:
\begin{enumerate}
\item \emph{Convolution}: Convolves the input with a filter, whose weights
are learned. The filter operates on all image channels, but only acts
on a small neighborhood of spatial pixels, determined by the kernel
size. Each filter takes as input a 3D image, and outputs a 2D image.
Each convolutional layer may have multiple filters, resulting in a
3D stack of filtered images as output. Assume the input is $X\in\mathbb{R}^{M_{in}\times N_{in}\times D_{in}}$.
Let $s_{k}$ be the kernel size (generally odd so that there is a
well-defined center) and $D_{out}$ be the number of filters. Then
the output of the convolutional layer is $Y\in\mathbb{R}^{M_{out}\times N_{out}\times D_{out}}$,
where $M_{out}=M_{in}-s_{k}+1$, $N_{out}=N_{in}-s_{k}+1$, and each
entry in $Y:=W\ast X$ is given by 
\[
Y_{ijk}=W_{0}^{k}+\sum_{r=1}^{D_{in}}\sum_{q=0}^{s_{k}}\sum_{p=0}^{s_{k}}W_{p,q,r}^{k}X_{i+p,j+q,r}
\]
where $W\in\mathbb{R}^{s_{k}\times s_{k}\times D_{in}\times D_{out}}$
and $W_{0}\in\mathbb{R}^{D_{out}}$ is a set of biases for each of
the $D_{out}$ filters.\\
In general, a zero padding of $s_{p}$ pixels can be introduced to
the spatial dimensions of the input image to change the output size.
This is particulary useful to make the output image the same size
as the input. Also, a stride of $s_{s}$ pixels can be used if it
is not desirable to apply filter to consecutive pixels. In this case,
$M_{out}=\frac{1}{s_{s}}(M_{in}-s_{k}+2s_{p})+1$ and $N_{out}=\frac{1}{s_{s}}(N_{in}-s_{k}+2s_{p})+1$
and
\[
Y_{ijk}=W_{0}^{k}+\sum_{r=1}^{D_{in}}\sum_{q=0}^{s_{k}}\sum_{p=0}^{s_{k}}W_{p,q,r}^{k}\tilde{X}_{s_{s}\cdot i+p,s_{s}\cdot j+q,r}
\]
where $\tilde{X}$ is the zero-padded image.\\
A common choice for kernel size is $s_{k}=3$, with zero padding $s_{p}=1$
and stride $s_{s}=1$. (Although this operation is actually known
as correlation in signal processing, the name \emph{convolution} has
stuck in the deep learning community).
\item \emph{Nonlinearity}: an element-wise nonlinear transformation that
allows neural networks to learn arbitrary functions. The most commonly
used is the rectified linear unit, aka ReLU. It is popular due to
its simplicity and has been shown emprically to improve training over
other functions, such as the sigmoid or tanh. Define $Y:=ReLU(X)$
where each entry 
\[
Y_{ijk}=\max(0,X_{ijk})
\]
\item \emph{Pooling}: Pooling is a (possibly) nonlinear downsampling of
the image, in order to reduce computational efforts and also allow
the model to be spatially invariant. The most common is max-pooling
with kernel size $2$ and stride $2$. This replaces each 2x2 patch
in the input with its max value:
\[
Y_{ijk}=\max_{p,q\in\{0,1\}^{2}}\left[X_{2\cdot i+p,2\cdot j+q,k}\right]
\]
For general kernel size $s_{k}$ and stride $s_{s}$, we have
\[
Y_{ijk}=\max_{p,q\in\{0,\dots,s_{k}\}^{2}}\left[X_{s_{s}\cdot i+p,s_{s}\cdot j+q,k}\right]
\]

\iffalse
\item \emph{Fully Connected}: Each output node of a fully connected layer
is simply an affine transformation of all nodes in the previous layer.
Let $D_{out}$ be the desired number of output nodes. Then $Y\in\mathbb{R}^{D_{out}}$
where each entry
\[
Y_{k}=W_{0}^{k}+\sum_{r=1}^{D_{in}}\sum_{q=1}^{N_{in}}\sum_{p=1}^{M_{in}}W_{pqr}^{k}X_{pqr}
\]
\item \emph{Softmax:} A transformation that normalizes the input across
the classes so that the output corresponds to a probability that each
pixel belongs to a certain class.
\[
P_{ijk}=\frac{\exp(X_{ijk})}{{\displaystyle \sum_{r=1}^{D_{in}}}\exp(X_{ijr})}
\]
Here $P_{ijk}$ is the probability that pixel $X_{ij}$ belongs to
class $k$.
\fi

\item \emph{Cross-Entropy Loss}: Let $L_{ij}\in\{0,\dots,C_{out}\}$ be
the true label of pixel $X_{ij}$. The cross-entropy loss is defined
as 
\[
-\sum_{ijk}{\bf 1}_{L_{ij}=k}\log(P_{ijk})
\]
where $\mathbf{1}$ is the indicator function.
\end{enumerate}

The CNN is trained by optimizing the weights of the network
so that the loss between the predicted and true labels are minimized
over the entire training set.




